Synthesizing Performance Constraints for Evaluating and Improving Code Efficiency

Large Language Models (LLMs) have been increasingly used to optimize code efficiency. Evaluating their effectiveness and further suggesting optimization opportunities often rely on high-quality tests to demonstrate the performance bottlenecks presented in the program. However, existing approaches rely on a limited set of hand-curated inputs or LLM-generated uninteresting length-stressing tests, failing to reveal more nuanced optimization opportunities. We present WEDGE, a framework for generating performance-stressing input given the program under test. WEDGE synthesizes explicit performance-characterizing constraints in the form of branch conditions to partition the programs' execution space into performance-specific regions. When integrated with the coverage-guided fuzzer, reaching different regions introduces explicit rewards for test generation to explore inefficient implementations. Our evaluation shows that WEDGE introduces a significant slowdown compared to the tests in CodeContests and those claimed to be optimized by existing approaches. From the utility perspective, integrating our tests substantially improves the existing code optimization approaches that rely on test-driven execution feedback. We release PERFFORGE, the performance tests generated by WEDGE, to benchmark future approaches for efficient code generation at https://github.com/UChiSeclab/perfforge.

==> dataset.tex <==
\section{\bench: A Benchmark for Code Efficiency Evaluation}

CodeContests contains over 3,000 problems (\codeforces section alone) with hundred of
    solutions which is far too large for an exhaustive analysis.
So, we apply three filters to obtain a manageable, yet 
    still meaningful benchmark. 
First, we exclude problems that execute $\leq$100,000 CPU
    instructions to ensure measurable performance variation.
Second, we remove problems that have less than ten solutions 
    or less than five inputs, to support effective fuzzing.
Third, we exclude problems that allow multiple correct solutions,
    to ensure a deterministic evaluation.
More details are provided in~\cref{appx:dataset-filtering}


==> experiments_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% New structure, but too much text (May'25) %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Experiments}

We evaluate \tool by (1) measuring the execution cost of \bench 
  the performance-exercising inputs generated by \tool (\cref{sec:quantitative_results}), 
  (2) investigating how useful these inputs are at 
  highlighting code inefficiencies (\cref{sec:tests-utility}), 
  and (3) conducting a comprehensive sensitivity 
  analysis (\cref{sec:sensitivity_analysis}).

\subsection{Setup}
\label{sec:setup}

\para{Dataset.} We evaluate \tool on the CodeContests~\cite{li-science22} dataset, 
  which covers a wide range of competitive programming problems and 
  human-written solutions. 
Test cases for these problems include the default inputs from the original dataset
  as well as additional inputs generated by~\alphacode~\cite{li-science22}. 
To ensure consistent and comparable performance measurements with other baselines
  (see below), we focus exclusively on C++ solutions. 

CodeContests contains over 3,000 problems with hunderds of C++ solutions 
  which is a far too large dataset for exhaustive analysis. 
  
Thus, we select a manageable yet comprehensive subset guided by three high-level 
  filtering criteria. 
First, to guarantee measurable performance variation, we exclude problems with 
  short-running solutions ($\leq$100K retired instrucitons). 
Second, to ensure adequate data for fuzzing, we require each problem to 
  have at least ten correct solutions and five tests inputs.  
Third, to focus on deterministic performance evaluation, we remove 
  any problem that allows multiple distinct correct outputs. 
Applying these criteria yields a shortlist that we then rank 
  by the execution time variation of their solution abd  select the top 300 problems. 
\tool successfully finds high-quality input pairs and generates constraints on 207 of them, 
  and after dropping those where baseline techniques produce no valid inputs, 
  we arrive at 154 problems spanning 33,020 C++ programs.

\para{Dataset.}

\para{Baselines.}
We evaluate performance-exercising efficiency of 
    \bench tests against the following benchmarks:

\textit{EvalPerf.} \evalperf~\cite{liu-colm24} develops a framework that leverages 
    an \llm to automatically  synthesize a parameterized input generator 
    that stresses code efficiency. 
It feeds the model a single reference solution to reason about 
    which inputs will slow that implementation down, and
    produces a test generator that progressively scales input size 
    until reaching a predefined threshold. 
Since our dataset doesn't have reference solutions per problem, 
    we compare \tool with two variants of \evalperf by selecting 
    either the slowest solution (\evalperfslow) or a random solution 
    (\evalperfrandom) as reference.

\textit{\directprompting.} To highlight the importance of asking the \llm to generate pc-constraints instead of directly generating the input itself (or an input generator), we also evaluate \tool against a stress-test generation approach similar to~\cite{du2024mercury}, \cite{peng2025coffecodeefficiencybenchmark}, and \cite{huang-neurips24-effibench}.
Specifically, we instruct the \llm to synthesize a program that generates performance-exercising inputs directly. 


We evaluate performance-exercising utility of \bench tests
    against the following benchmarks:

\textit{EffiLearner.} \effilearner~\cite{huang-neurips24} is a self-optimization framework that uses 
  running time and memory profiling to guide an \llm in refining its own code. 
It generates a program implementing a particular specification, 
  executes it locally to capture overhead data, then feeds those profiles 
  back into the model to iteratively reduce performance bottlenecks.
\effilearner pinpoints hotspot lines and memory-intensive operations 
    by instrumenting each run, then crafts targeted prompts 
    that instruct the \llm to refactor inefficient 
    code constructs (e.g., nested loops, redundant data structures).


\textit{Performance improving edits.} \pie~\cite{shypula-iclr24} is a framework that leverages an LLM trained on human 
  C++ performance-improving edits.
\pie modifies code by iteratively steering the language model towards a 
  desired performance target (e.g., ``2$\times$ speedup'')
  by iteratively presenting the LLM code edits with their 
  annotated speedup.



\para{Metrics} \para{Metrics.} To measure performance, 
    we rely on the number of (retired) instructions 
    based and physical execution time.
We use the \texttt{perf} Linux utility~\cite{weaver2013linux} 
    for both measurements.
While physical running time is a more intuitive measurement, 
    it can be prone to 
    interference from transient system effects—such as background 
    processes, scheduling policies, 
    and variable I/O latencies—which may mask true computational 
    cost~\cite{de2010new,zhang-eurosys13}.  
In contrast, measuring instruction counts is a metric that is more stable across run, platform-agnostic, 
  and is well understood to significantly correlate with executions 
  exhibiting performance bottlenecks~\cite{curtsinger-sosp15,zhang-eurosys13,iorgulescu-atc18,delimitrou-asplos14}.
Recently, LLM-informed code analysis tools started to rely on instruction count measured through 
  hardware counters~\cite{liu-colm24, peng2025coffecodeefficiencybenchmark} or emulation~\cite{shypula-iclr24} 
  to evaluate code efficiency as it provides a more reliable, low-variance 
  measurement than physical time alone.
Moreover, experiments in~\cite{peng2025coffecodeefficiencybenchmark} 
    mirror our findings (Table~\cref{tab:efficiency-instruction-count} that 
    instruction count measurements are two orders of magnitude more 
    more stable than physical execution time, 
    which mirrors our findings (see \cref{tab:} and \cref{fig:}).


\subsection{Efficiency of \bench}
\label{sec:quantitative_results}



To determine the efficiency of \bench we run each 
    solution for each problem against the generated tests 
    and compare the number of instructions executed against
    the \evalperf and \directprompting baselines.
To reduce noise, we run each program five times, and 
    compute the average instruction counts for those runs.
We then compute the average of those values across all 
    programs and all problems.
While \bench includes top ten tests triggering slowdown 
    generated by \tool, we further include comparisons for 
    top five, top three, and topmost inputs triggering
    execution slowdown, respectively, to illustrate the 
    robustness of our performance-stress 
    test generation technique.
    
As Table~\ref{tab:efficiency-instruction-count} shows, 
    \bench tests lead the programs executing between 
    $2\times$ more instructions, on average, 
    when compared to the state of the art.
\evalperf, while efficient, is optimized to focus 
    on inputs close to the upper bound of the problem 
    statement constraints (see~\cref{appx:case-studies}).

\tool also outperforms direct prompting, albeit 
    by a smaller margin.
Direct prompting is designed to synthesize an input
    generator by taking into acount the problem specification 
    and constraints, similar to~\cite{peng2025coffecodeefficiencybenchmark, huang-neurips24, du2024mercury}.
We manually analyze a sample of these generators 
    (\cref{appx:case-studies}).
While the \llm attempts to implicitly reason about 
    how to stress-test programs by inferring 
    more diverse input patterns, these are ultimately 
    focused on generic patterns specific to the 
    broader class of algorithms that the problem 
    implements (e.g., large graphs for graph-based problems).
Consequently, there is little guarantee
    that these patterns reveal more complex performance 
    bottlenecks.
    


Appendix~\cref{sec:appendix-running-time} shows a similar
    trend when comparing each technique head-to-head
    while measuring physical running time.
However, the measurement variance is more significant, 
    reaching $12\%$.
While multiple factors contribute to this large variance,
    we argue that the dominant factor of ``noise'' is I/O 
    as a sizable fraction of programs 
    need to read thousands of KB, thus making them 
    I/O-bound.

Note that these results are not dominated 
    by a few outliers.
Rather, \bench tests are robust.
This is best illustrated in 
    \cref{fig:slowdown-distrubution}
    where we plot the raw instruction count for 
    every program across all problems 
    as a cumulative distribution.
Tests in \bench consistently induce 
    larger slowdowns across the aggregated 
    set of programs.

As further support of this, 
    \cref{fig:histogram_head_to_head} 
    plots a series of histograms where we compare \tool 
    and all other baselines.
Specifically, We count how many programs 
    are slower when using our tests versus tests generated 
    by the other techniques.
We then divide this numbers in buckets of 10\% size.
A positive percentage indicates that \bench tests induce 
    more slowdown, while a negative percentage indicates 
    that the other technique in the head-to-head comparison
    does.
So, higher bars in the right side of each graph indicate 
    \tool outperforms that particular baseline.


% \begin{table*}[!t]

%     \centering
%     \setlength{\tabcolsep}{5pt}
%     \renewcommand{\arraystretch}{1}
%     \small

%   \caption{Comparison between \tool and baseline techniques, after removing inputs that run for 
%   more than 60sec (KILL). Average \#instructions ($\times 10^8$) and relative slowdown compared with default tests across all tested programs running top-$k$, $k={10, 5, 3, 1}$ slowest inputs.
%   \label{tab:efficiency-instruction-count}


% \begin{tabular}{lllll}
% \toprule
% Technique & \bench & \bench$_{t5}$ & \bench$_{t3}$ & \bench$_{t1}$ \\ \midrule
% wedge & \textbf{5.19$\pm$0.03\%} & \textbf{5.42$\pm$0.03\%} & \textbf{5.62$\pm$0.03\%} & \textbf{6.00$\pm$0.03\%} \\
% direct-prompt & 3.70$\pm$0.03\% (\textcolor{red}{$\downarrow$}1.4$\times$) & 4.21$\pm$0.02\% (\textcolor{red}{$\downarrow$}1.3$\times$) & 4.52$\pm$0.02\% (\textcolor{red}{$\downarrow$}1.2$\times$) & 5.14$\pm$0.02\% (\textcolor{red}{$\downarrow$}1.2$\times$) \\
% evalperf-rand & 2.66$\pm$0.03\% (\textcolor{red}{$\downarrow$}2.0$\times$) & 3.50$\pm$0.03\% (\textcolor{red}{$\downarrow$}1.5$\times$) & 3.93$\pm$0.03\% (\textcolor{red}{$\downarrow$}1.4$\times$) & 4.31$\pm$0.03\% (\textcolor{red}{$\downarrow$}1.4$\times$) \\
% evalperf-slow & 2.57$\pm$0.03\% (\textcolor{red}{$\downarrow$}2.0$\times$) & 3.40$\pm$0.03\% (\textcolor{red}{$\downarrow$}1.6$\times$) & 3.82$\pm$0.02\% (\textcolor{red}{$\downarrow$}1.5$\times$) & 4.24$\pm$0.02\% (\textcolor{red}{$\downarrow$}1.4$\times$) \\
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}[!t]

%     \centering
%     \setlength{\tabcolsep}{5pt}
%     \renewcommand{\arraystretch}{1}
%     % \small

%   \caption{Comparison between \tool and baseline techniques, after filtering out long-running 
%   invalid inputs}

% \begin{tabular}{lllrrr}
% \toprule
% \multirow{2}{*}{Technique} & \multicolumn{2}{c}{\#instructions ($\times 10^8$)} & \multirow{2}{*}{Win rate} & \multicolumn{2}{c}{Rel. to AlphaCode} \\
%               & \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median} & & \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median} \\
% \midrule
% \textbf{Baselines}\\
% wedge & \textbf{5.73} & \textbf{0.60} & \textbf{59\%} & \textbf{4.8$\times$} & \textbf{77.9$\times$} \\
% tg-prompt & 3.74 (\textcolor{red}{$\downarrow$}1.5$\times$) & 0.52 (\textcolor{red}{$\downarrow$}1.2$\times$) & 15\% & 3.2$\times$ & 66.8$\times$ \\
% evalperf-slow & 3.13 (\textcolor{red}{$\downarrow$}1.8$\times$) & 0.37 (\textcolor{red}{$\downarrow$}1.6$\times$) & 13\% & 2.6$\times$ & 48.5$\times$ \\
% evalperf-rand & 3.11 (\textcolor{red}{$\downarrow$}1.8$\times$) & 0.39 (\textcolor{red}{$\downarrow$}1.5$\times$) & 13\% & 2.6$\times$ & 50.6$\times$ \\
% \midrule
% \textbf{Ablations}\\
% wedge-yesInstr-defaultMut & 2.87 (\textcolor{red}{$\downarrow$}3.0$\times$) & 0.01 (\textcolor{red}{$\downarrow$}48.0$\times$) & xx\% & 0.40 & 1.07 \\
% wedge-noInstr-constrntMut & 8.63 (1.0$\times$) & 0.09 (\textcolor{red}{$\downarrow$}3.8$\times$) & xx\% & 0.13 & 0.08 \\
% wedge-noInstr-defaultMut & 3.30 (\textcolor{red}{$\downarrow$}2.6$\times$) & 0.01 (\textcolor{red}{$\downarrow$}48.0$\times$) & xx\% & 0.35 & 1.07 \\
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{table*}[!t]

    \centering
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1}
    % \small

  \caption{[FINAL-INSTR-COUNT] \tool versus baseline techniques, after filtering out long-running 
  invalid inputs}

\begin{tabular}{lllrrr}
\toprule
\multirow{2}{*}{Technique} & \multicolumn{2}{c}{\# of instructions} & \multirow{2}{*}{Win rate} & \multicolumn{2}{c}{Rel. to AlphaCode} \\
              & \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median} & & \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median} \\
\midrule
wedge & 5.96 & 0.75 & 59.3\% & 363.07 & 0.01 \\
evalperf-slow & 3.23 (\textcolor{red}{$\downarrow$}1.8$\times$) & 0.44 (\textcolor{red}{$\downarrow$}1.7$\times$) & 11.9\% & 146.48  & 0.02 \\
evalperf-rand & 3.21 (\textcolor{red}{$\downarrow$}1.9$\times$) & 0.45 (\textcolor{red}{$\downarrow$}1.7$\times$) & 13.6\% & 166.06 & 0.02 \\
direct-prompt & 3.87 (\textcolor{red}{$\downarrow$}1.5$\times$) & 0.60 (\textcolor{red}{$\downarrow$}1.3$\times$) & 15.2\% & 274.66 & 0.01 \\
\bottomrule
\end{tabular}

\end{table*}

\begin{table*}[!t]

    \centering
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1}
    % \small

  \caption{[FINAL-RUN-TIME] \tool versus baseline techniques, after filtering out long-running 
  invalid inputs}

\begin{tabular}{lllrrr}
\toprule
\multirow{2}{*}{Technique} & \multicolumn{2}{c}{Running time (ms)} & \multirow{2}{*}{Win rate} & \multicolumn{2}{c}{Rel. to AlphaCode} \\
              & \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median} & & \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median} \\
\midrule
wedge & 228.60 & 82.33 & 59.3\% & 1.65 & 0.09 \\
evalperf-slow & 139.83 (\textcolor{red}{$\downarrow$}1.6$\times$) & 61.69 (\textcolor{red}{$\downarrow$}1.3$\times$) & 11.9\% & 0.95 & 0.01 \\
evalperf-rand & 134.79 (\textcolor{red}{$\downarrow$}1.7$\times$) & 60.90 (\textcolor{red}{$\downarrow$}1.4$\times$) & 13.6\% & 0.98 & 0.01 \\
direct-prompt & 182.15 (\textcolor{red}{$\downarrow$}1.3$\times$) & 85.60 (\textcolor{green}{$\uparrow$}1.0$\times$) & 15.2\% & 1.40 & 0.01 \\
\bottomrule
\end{tabular}

\end{table*}

\begin{table*}[!t]

    \centering
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1}
    % \small

  \caption{[FINAL-INSTR-COUNT] \tool versus ablated versions, after filtering out long-running invalid inputs}

\begin{tabular}{lllrrr}
\toprule
\multirow{2}{*}{Technique} & \multicolumn{2}{c}{\# of instructions} & \multirow{2}{*}{Win rate} & \multicolumn{2}{c}{Rel. to AlphaCode} \\
              & \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median} & & \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median} \\
\midrule
wedge & 5.96 & 0.75 & 64.8\% & 363.07 & 0.01 \\
wedge-yesInstr-defaultMut & 1.54 (\textcolor{red}{$\downarrow$}3.9$\times$) & 0.01 (\textcolor{red}{$\downarrow$}102.9$\times$) & 3.6\% & 11.69 & 0.09 \\
wedge-noInstr-constrntMut & 4.02 (\textcolor{red}{$\downarrow$}1.5$\times$) & 0.21 (\textcolor{red}{$\downarrow$}3.6$\times$) & 29.2\% & 159.23 & 0.04 \\
wedge-noInstr-defaultMut & 1.49 (\textcolor{red}{$\downarrow$}4.0$\times$) & 0.01 (\textcolor{red}{$\downarrow$}103.0$\times$) & 2.4\% & 30.03 & 0.09 \\
\bottomrule
\end{tabular}

\end{table*}


\begin{table*}[!t]

    \centering
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1}
    % \small

  \caption{[FINAL-RUN-TIME] \tool versus ablated versions, after filtering out long-running 
  invalid inputs}

\begin{tabular}{lllrrr}
\toprule
\multirow{2}{*}{Technique} & \multicolumn{2}{c}{Running time (ms)} & \multirow{2}{*}{Win rate} & \multicolumn{2}{c}{Rel. to AlphaCode} \\
              & \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median} & & \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median} \\
\midrule
wedge & 228.60 & 82.33 & 64.8\% & 1.65 & 0.09 \\
wedge-yesInstr-defaultMut & 86.57 (\textcolor{red}{$\downarrow$}2.6$\times$) & 59.13 (\textcolor{red}{$\downarrow$}1.4$\times$) & 3.6\% & 0.52 & 0.01 \\
wedge-noInstr-constrntMut & 171.63 (\textcolor{red}{$\downarrow$}1.3$\times$) & 71.54 (\textcolor{red}{$\downarrow$}1.2$\times$) & 29.2\% & 1.20 & 0.01 \\
wedge-noInstr-defaultMut & 78.27 (\textcolor{red}{$\downarrow$}2.9$\times$) & 45.13 (\textcolor{red}{$\downarrow$}1.8$\times$) & 2.4\% & 0.47 & 0.01 \\
\bottomrule
\end{tabular}


\end{table*}



We manually inspect several cases where \tool tests significantly outperform baseline tests and make the following observations.
One notable example is \codeforces Problem 633A (Figure~\ref{fig:motivating}), where \tool tests significantly outperform \evalperfrandom, \evalperfslow, \directprompting tests.
We defer a detailed analysis to~\cref{appx:motivating-example}.


% \begin{figure*}[!t]

% \centering

% \subfloat[\tool vs.\evalperfslow]{
%         \includegraphics[width=0.24\linewidth]{figures/areachart_wedge_vs_evalperf-slow_top10inputs.pdf}
%         \label{subfig:areachart_wedge_vs_evalperf-slow_top10inputs}
%     }
% \subfloat[\tool vs.\evalperfrandom]{
%         \includegraphics[width=0.24\linewidth]{figures/areachart_wedge_vs_evalperf-rand_top10inputs.pdf}
%         \label{subfig:areachart_wedge_vs_evalperf-rand_top10inputs}
%     }
% \subfloat[\tool vs.\directprompting]{
%         \includegraphics[width=0.24\linewidth]{figures/areachart_wedge_vs_direct-prompt_top10inputs.pdf}
%         \label{subfig:areachart_wedge_vs_direct-prompt_top10inputs}
%     }
    
% \caption{
% \label{fig:slowdown-distrubution}
% \end{figure*}




\begin{figure*}[!t]

\centering

\captionsetup[subfigure]{labelformat=empty,font=small}

\subfloat[vs.\evalperfslow (top-10)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-slow_top10inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-slow_top10inputs}
    }
\subfloat[vs.\evalperfslow (top-5)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-slow_top5inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-slow_top5inputs}
    }
\subfloat[vs.\evalperfslow (top-3)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-slow_top3inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-slow_top3inputs}
    }
\subfloat[vs.\evalperfslow (top-1)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-slow_top1inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-slow_top1inputs}
    }

\subfloat[vs.\evalperfrandom (top-10)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-rand_top10inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-rand_top10inputs}
    }
\subfloat[vs.\evalperfrandom (top-5)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-rand_top5inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-rand_top5inputs}
    }
\subfloat[vs.\evalperfrandom (top-3)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-rand_top3inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-rand_top3inputs}
    }
\subfloat[vs.\evalperfrandom (top-1)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-rand_top1inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-rand_top1inputs}
    }

\subfloat[vs.\directprompting (top-10)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_direct-prompt_top10inputs.pdf}
        \label{subfig:histogram_wedge_vs_direct-prompt_top10inputs}
    }
\subfloat[vs.\directprompting (top-5)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_direct-prompt_top5inputs.pdf}
        \label{subfig:histogram_wedge_vs_direct-prompt_top5inputs}
    }
\subfloat[vs.\directprompting (top-3)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_direct-prompt_top3inputs.pdf}
        \label{subfig:histogram_wedge_vs_direct-prompt_top3inputs}
    }
\subfloat[vs.\directprompting (top-1)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_direct-prompt_top1inputs.pdf}
        \label{subfig:histogram_wedge_vs_direct-prompt_top1inputs}
    }

\caption{Comparisons between \tool (\textcolor{CustomOrange}{\ding{110}}) and the other baselines (\textcolor{CustomPurple}{\ding{110}}). The bars represent the number of programs where one of the tools incurs a larger instruction count when running over the top-$k$ ($k=\{1,3,5,10\}$) slowest inputs generated by our tool.
\label{fig:histogram_head_to_head}

\end{figure*}


\subsection{Utility of \bench}
\label{sec:tests-utility}


Execution feedback has proven valuable for LLM-based code 
    edits~\cite{chunqiu-issta24,peng2024perfcodegen,huang-neurips24}.
However, its effectiveness hinges on tests that accurately expose 
    performance bottlenecks.
Such effectivness relies on high-quality tests that are 
    capable of surfacing performance bottlenecks.
We investigate the utility of \bench by using our generated tests 
  to provide feedback to two state-of-the-art \llm-based 
  code optimization tools: 
  \effilearner~\cite{huang-neurips24} and 
  \pie~\cite{shypula-iclr24}.

\subsubsection{Code optimization with execution feedback}

Building on the \effilearner workflow, we first collect a 
  corpus of 280 slow Python solutions from a subset 56 problems 
  of our original dataset (see Appendix A for filtering details)
  
For each solution, we run the original public test suite
  that \effilearner uses and compare it with \bench. 
Following their original evaluation methodology, 
  we profile each run and record phyisical execution time and 
  memory consumption statistics.

Next, we convert these raw traces into the same 
  prompt format described by the paper,
  as a summary of the top bottleneck functions 
  annotated with the corresponding metrics.
We then prompt the model with three different variants:
\begin{enumerate}
  \item \textit{No profile}: the solution code alone, 
    without any profiling data.
  \item \textit{Default profile}: code plus profiling summary 
    from the original default tests.
  \item \textit {\bench profile}: code plus profiling summary 
    derived from our \bench tests.
\end{enumerate}


\begin{table*}[!t]
    \centering
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1}
    \small

    \caption{EffiLearner Experiment 
    \label{tab:effilearner-experiment}
    \begin{tabular}{rlr|r|r|r}
        \toprule
        \textbf{Model} & \textbf{Test Input Set} & \makecell{\textbf{Execution} \\ \textbf{Time (s)}} &
        \makecell{\textbf{Total Memory} \\ \textbf{Usage (Mb * s)}} &
        \makecell{\textbf{Max Memory} \\ \textbf{Usage (Mb)}} &
        \makecell{\textbf{Execution} \\ \textbf{Time (\#inst)}} \\
        \midrule
        \multirow{3}{*}{GPT-4o} 
          & no\_profile     & 15.66\%              & 21.70\%         & 2.78\%           & 31.39\% \\
          & public\_profile & 22.57\%              & 27.78\%         & \textbf{11.89\%} & 39.89\% \\
          & wedge\_profile  & \textbf{26.47\%}     & \textbf{35.10\%}& 11.82\%          & \textbf{49.31\%} \\ 
        \midrule
        \multirow{3}{*}{DeepSeek-V3} 
          & no\_profile     & 6.77\%               & 12.49\%         & 2.30\%           & 20.48\% \\
          & public\_profile & 12.29\%              & 20.43\%         & 1.93\%           & 35.01\% \\
          & wedge\_profile  & \textbf{18.99\%}     & \textbf{23.75\%}& \textbf{9.21\%}  & \textbf{40.26\%} \\ 
        \bottomrule
    \end{tabular}
\end{table*}

We measure the utility of \bench for optimizing code 
    using two models, OpenAI GPT-4o and DeepSeek V3,
    
We apply the same prompting strategies, structure, and 
    formatting as in the original paper~\cite{huang-neurips24-effibench}.
Finally we mirror the same metrics as \effilearner, namely
    physical execution time, total memory utilization,
    and maximum memory usage, and we add 
    instruction count as an additional measurement.

Table~\ref{tab:effilearner-experiment} illustrates that using
    \bench tests leads to more performance improvement.

\effilearner can optimize the code to execute 
    24\% less instructions (or approximately 
    10 percentage points), run 17\% faster and use 
    25\% less memory on average when providing GPT-4o 
    with \bench execution profiles as opposed to 
    their original setup.
Similarly, \effilearner can optimize the code to execute
    15\% less instructions, run 46\% faster and use 
    16\% less memory when providing DeepSeek with the 
    same \bench-backed execution profiles.

\subsubsection{Code optimization models}

We further investigate the utility of \bench,
    by evaluating performance improvement gains on 
    language models fine-tuned for code optimization, 
    in addition to LM-backed feedback-driven code optimizations.
To this end, we evaluate our generate tests on 
    \pie~\cite{shypula-iclr24}, a state-of-the-art 
    LM-informed code optimization technique.
We select the three most effective models presented by 
    the paper (1) ..., (2), ..., (3) ... .
We then adapt our problem selection to match the requirements 
    of \pie, and include two aditional filtering policies 
    on top of those in~\cref{sec:eval-setup}. 
First, we keep only programs short enough,
    i.e., $\leq50$ SLoCs, to fit the context 
    window of the three models.
Second, we retain only solutions that are suboptimal, 
    i.e., at least twice as slow as the fastest solution
    for that particular problem,
    so that there is space for code improvements 
    than the fastest solution.

We use a similar set of metrics as~\cite{shypula-iclr24}. 
Specifically, we measure the average relative 
    speedup between the original and optimized programs 
    in terms of instruction counts and physical time,
    as well as the percentage of programs that the \llm 
    models can \textit{meaningfully} optimize by 
    more than 10\%~\cite{shypula-iclr24}.

Table~\cref{tab:pie-experiment} illustrates how our 
   tests are better at highlighting performance bottlenecks.
\bench outperforms the other techniques by 24\% to 149\% in 
    terms of instruction counts and by 5\% to 27\% in terms 
    of physical time.
It also help discover that between 7\% and 48\% more programs 
    have actually been meaningfully optimized 
    and run at least 10\% faster.


\begin{table*}[!t]

    \centering
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1}
    \small

  \caption{Pie Experiment}
  \label{tab:pie-experiment}
\begin{tabular}{rlrrrr}
\toprule
\textbf{Model} & \textbf{Test Input Set} & \multicolumn{1}{l}{\textbf{Speedup (\#inst)}} & \multicolumn{1}{l}{\textbf{Speedup (time)}} & \multicolumn{1}{l}{\textbf{\%Opt (\#inst)}} & \multicolumn{1}{l}{\textbf{\%Opt (time)}} \\ \midrule
\multirow{3}{*}{\piehq} & \defaultall & 1.32 & 0.93 & 6.03\% & 16.58\% \\
 & \defaultslowfive & 1.30 & 0.94 & 5.53\% & 18.09\% \\
 & \wedgeslowfive & \textbf{1.62} & \textbf{1.18} & \textbf{12.06\%} & \textbf{26.63\%} \\ \midrule
\multirow{3}{*}{\piecond} & \defaultall & 1.98 & 1.13 & 16.23\% & 29.22\% \\
 & \defaultslowfive & 1.85 & 1.13 & 15.58\% & 27.92\% \\
 & \wedgeslowfive & \textbf{1.99} & \textbf{1.29} & \textbf{18.83\%} & \textbf{41.56\%} \\ \midrule
\multirow{3}{*}{\pieuncond} & \defaultall & 1.21 & 1.32 & 4.35\% & 56.52\% \\
 & \defaultslowfive & 1.21 & 1.32 & 4.35\% & 56.52\% \\
 & \wedgeslowfive & \textbf{3.01} & \textbf{1.38} & \textbf{30.43\%} & \textbf{60.87\%} \\ \bottomrule
\end{tabular}
\end{table*}

\subsection{Sensitivity Analysis}
\label{sec:sensitivity_analysis}
\subsubsection{Ablations}

To understand the impact of our design
    choice, we ablate the two key decisions: 
    (1) involving pc-constraints
    in mutator generation, 
    (2) instrumenting the original 
    program with \textit{constraint checker} code.
For (1), we use a \textit{constraint-agnostic} 
    mutator for comparison.
The constraint-aware mutator and 
    constraint-agnostic mutator are generated by prompting with and without the 
    pc-constraints.
For (2), we use the original program for comparison.

Table~\ref{tab:ablation} shows the performance of \tool and ablated versions.
\tool tests (using top-10 inputs) are on average 63.03\% and 62.34\% slower (in terms of relative slowdown and \#instructions) than \wedgenoinstrument.
The results show using instrumented programs (programs with constraint checkers inserted) can provide guidance to fuzzing, thus generating slower tests compared with not inserting the checkers.
Similarly, \wedgenoinstrument tests are on average 155.17\% and 156.99\% slower than \wedgenoconstraint.
On 63.02\% solutions \wedgenoinstrument tests are slower (with a significance value of 0.05, according to Mann-Whitney test~\cite{mcknight2010mann}).
This underscores the importance of the performance-constraint-aware mutator.

\begin{table}
\centering
\small
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.1}
\caption{Comparison between \tool and ablated versions. We report relative slowdown compared with default tests and average instruction count ($\times 10^8$) across all tested programs using the top-$k$ slowest inputs ($k=10, 5, 3, 1$).
\label{tab:ablation}
% \begin{tabular}{lllll}\toprule \# of slowest inputs & Top-10 & Top-5 & Top-3 & Top-1 \\ \midrule
% \rowcolor[gray]{0.95} \multicolumn{5}{c}{Relative slowdown compared with default tests} \\
%  \wedgenoconstraint & 242.16 & 365.37 & 424.16 & 423.97  \\ \wedgecustom & 342.98 & 442.40 & 458.79 & 457.04  \\ \wedgenoinstrument & 391.93 & 472.51 & 561.46 & 703.19  \\ \toolfull & \textbf{513.21} & \textbf{594.58} & \textbf{654.49} & \textbf{803.62}  \\ \midrule
% \rowcolor[gray]{0.95} \multicolumn{5}{c}{Number of instructions ($\times 10^8$)} \\
%  \wedgenoconstraint & 3.00 & 4.05 & 4.69 & 5.07  \\ \wedgecustom & 3.95 & 4.89 & 5.18 & 5.64  \\ \wedgenoinstrument & 5.29 & 6.12 & 6.98 & 8.91  \\ \toolfull & \textbf{6.58} & \textbf{7.45} & \textbf{8.19} & \textbf{10.66}  \\ \bottomrule
% \end{tabular}
\begin{tabular}{lllll}\toprule \# of slowest inputs & Top-10 & Top-5 & Top-3 & Top-1 \\ \midrule
\rowcolor[gray]{0.95} \multicolumn{5}{c}{Relative slowdown compared with default tests} \\
 \wedgenoconstraint & 240.80 & 363.33 & 421.79 & 421.60  \\ \wedgecustom & 341.06 & 439.93 & 456.22 & 454.49  \\ \wedgenoinstrument & 389.74 & 469.87 & 558.32 & 699.25  \\ \toolfull & \textbf{510.34} & \textbf{591.26} & \textbf{650.83} & \textbf{799.12}  \\ \midrule
\rowcolor[gray]{0.95} \multicolumn{5}{c}{Number of instructions ($\times 10^8$)} \\
 \wedgenoconstraint & 2.99 & 4.03 & 4.66 & 5.04  \\ \wedgecustom & 3.92 & 4.87 & 5.15 & 5.61  \\ \wedgenoinstrument & 5.27 & 6.09 & 6.94 & 8.86  \\ \toolfull & \textbf{6.55} & \textbf{7.41} & \textbf{8.15} & \textbf{10.60}  \\ \bottomrule
\end{tabular}


\end{table}


\begin{table}

\caption{Ablations numbers collected by Bogdan}

\begin{tabular}{lllrrr}
\toprule
\multirow{2}{*}{Technique} & \multicolumn{2}{c}{\# of instructions} & \multirow{2}{*}{Win rate} & \multicolumn{2}{c}{Rel. to AlphaCode} \\
              & \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median} & & \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median} \\
\midrule
wedge & 8.62 & 0.34 & xx\% & 0.13 & 0.02 \\
wedge-yesInstr-defaultMut & 2.87 (\textcolor{red}{$\downarrow$}3.0$\times$) & 0.01 (\textcolor{red}{$\downarrow$}48.0$\times$) & xx\% & 0.40 & 1.07 \\
wedge-noInstr-constrntMut & 8.63 (1.0$\times$) & 0.09 (\textcolor{red}{$\downarrow$}3.8$\times$) & xx\% & 0.13 & 0.08 \\
wedge-noInstr-defaultMut & 3.30 (\textcolor{red}{$\downarrow$}2.6$\times$) & 0.01 (\textcolor{red}{$\downarrow$}48.0$\times$) & xx\% & 0.35 & 1.07 \\
\bottomrule
\end{tabular}

\end{table}


\subsubsection{Effect of constraints.}

\para{Discrimination of performance-characterizing constraints.}
To investigate whether and how \tool generated performance-characterizing constraints can classify inputs, we select a set of 813 solution programs where both constraint-satisfying inputs and constraint-violating inputs exist.
We compare the average \#instructions of both sets on each solution.
Constraint-satisfying inputs are on average 51.46$\times$ slower than constraint-violating inputs.
We conduct a Mann-Whitney test~\cite{mcknight2010mann}, and constraint-satisfying inputs are significantly slower (with a significance value p < 0.05) than constraint-violating inputs on 93.73\% solution programs.
It demonstrates the performance-characterizing constraints generated by \tool are discriminative across most programs.

\para{Impact of constraints in guiding fuzzing.}
To better understand the impact of guidance of constraints (including mutator and fuzz driver instrumentation), we calculate the ratio of constraint-satisfying inputs (out of valid inputs) per strategy.
The result shows involving performance-constraints and constraint-checking branches contribute positively to the ratio of constraint-satisfying inputs.
Specifically, the ratios of constraint-satisfying inputs among generated inputs of \wedgenoconstraint, \wedgenoinstrument, and \tool are 49.11\%, 77.62\% and 80.48\% respectively.

\subsubsection{Effect of input size}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Old structure (Apr'25) %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Experiments}
\label{sec:eval}

We evaluate \tool by (1) comparing the execution cost of the performance-stressing inputs it generates, aggregated under the \bench benchmark, with the baselines (\cref{sec:quantitative_results}); (2) comparing \tool with the ablated versions where some design choices of \tool are disabled to show the contribution of each design choice; and (3) the utility of \bench inputs in terms of evaluating and improving \llm-based code optimization techniques (\cref{sec:tests-utility}).
% In \cref{sec:ablations}, we study how the performance-characterizing constraints generated by \tool help in each of its design choices.

\subsection{Setup}
\label{sec:setup}

\para{Dataset.} We run \tool on the CodeContests dataset~\cite{li-science22}, a large-scale collection of competitive programming problems and their associated human-written solutions.
This dataset spans multiple online judge platforms and encompasses a broad range of algorithmic and data-structure challenges. Each problem includes a set of solutions, some correct and others incorrect, written in languages such as C, C++, Java, and Python. 
Test inputs are included to check functional correctness.
In addition to public and private tests provided by \codeforces platform, a set of tests generated by the model trained by \citet{li-science22} are also included.
% In this paper we focus only on C++ solutions which comprise above 75\% of the dataset.
% 
We focus only on C++ solutions since C++ provides more predictable performance compared with other interpreted languages with runtime optimizations (JIT compilation in Python/Java), and it is widely used by many performance-critical applications, \eg high-frequencey trading.

\iffalse
Even when generating the most challenging inputs, not every program in the original dataset can exhibit meaningful performance variation (e.g., the program might implement the optimal or near-optimal solution for the given problem). 
As such, we focus on problems and programs in the original CodeContests dataset that exibith performance diversity and exeuction time variation by applying a series of filters to prune out potentially uninformative programs.

\noindent---\textit{Sufficient Computation.} We remove problems whose solutions never exceed 10,000 instructions on any input. 

\noindent---\textit{Sufficient tests.}We remove problems with fewer than five correct solutions or fewer than five test inputs (sufficient data). 

\noindent---\textit{Output agreement.} We filter out problems that accept multiple correct outputs.
We rely on having a ground-truth output to filter out the model's potential confabulation during pc-constraint generation and source code instrumentation.
As such, we remove any problems where less than 95\% of solutions agree on outputs for the provided test cases. 
\fi

Note that the \codecontest dataset (``train'' split, \codeforces problems) alone contains 3834 problems.
It is not feasible to evaluate all 3000+ problems.
We apply the following filters:
(1) \textit{Sufficient computation.} We remove problems whose solutions never exceed 100,000 instructions on any input to reduce the impact of potential noise following \citet{liu-colm24}.
(2) \textit{Sufficient solutions.} We remove problems with fewer than 10 correct solutions.
Because we later need to run fuzzing on sufficient correct solutions.
(3) \textit{Sufficient test inputs.} We remove problems with fewer than 5 default tests.
Because we need sufficient inputs to mine input pairs.
(4) \textit{Single output.} We filter out problems that accept multiple correct outputs.
(5) \textit{Diversified performance.} We only include problems with diversified performance across the solutions. 
Specifically, we use Coefficient of Variance (CV) to measure the diversity.
Low diversity means most solutions have similar performance, indicating the solutions are likely optimal or close to optimal.
Intuitively there are less opportunities to identify performance-characterizing constraints on the optimal solutions.
Therefore, we prefer the problems where there are more suboptimal or non-performant solutions.
We first apply the above five filters on 3,834 problems.
Then we rank the problems based on the CV and select the top 300 problems.
On 207 out of the 300 problems \tool can find at least one high-quality input pair and generate constraints.
For a fair comparison, we remove the problems where the baseline techniques fail to generate any valid inputs, leading to a set of 153 problems where all evaluated techniques generate at least one valid input.
We only include the solutions labeled as ``correct'' by the \codeforces platform.
In addition, we use the tests provided by \codecontest dataset to perform a sanity check, \ie removing the false positive solutions with the additional tests following \citet{li-science22}.
The 153 problems along with 32,835 solutions constitute our main evaluation dataset.
% 

% This sequence of filters yields 933 problems ().
% We then follow a methodology similar to ~\cite{liu-colm24} to select the most ``computationally meaningful'' programs of our data set.
% Specifically, we run each of the solutions of the 933 problems on a set of tests generated by a state of the art language model based test generator, AlphaCode~\cite{li-science22}, and rank those problems based on the coefficient of variation (CV) of running times and select the top 300 problems such that our total dataset of close to 20,000 C/C++ programs.

\para{Baselines.} We evaluate \tool against the following set of baselines.

\textit{EvalPerf.} \evalperf~\cite{liu-colm24} develops a state-of-the-art stress test generation technique that aims to rigorously assess code efficiency through prompting an \llm with CoT few-shot learning to produce a scale-controllable test input sampler.
% The key idea of \evalperf is to ask a language model to ``synthesize a (test) synthesizer'' that would o automatically produce performance-exercising inputs of a set of diverse programming tasks.
% \evalperf starts with a set of programming tasks and a set of programs that implement solutions to those tasks.
% It prompts the language model to ``synthesize a (test) synthesizer'' by providing the task description and works in two settings: either the slowest program that (\evalperfslow), or randomly chosen program that impelemts that programming task (\evalperfrandom).
% We compare the efficacy of \tool's generate tests to that of \evalperfslow and \evalperfrandom
\evalperf prompts an \llm by providing an example solution program (reference solution) and instructing it to reason what kind of inputs can make the program run slow.
It will produce a generator function with a parameter \codeIn{scale} that characterize the input size.
It then samples concrete test inputs from these generators, starting with a scale factor of 2 and increasing it exponentially until hitting the 20-second time wall or the 16GB memory wall.
As \codecontest does not contain reference solutions, we use a random solution and the slowest solution respectively as the example solution in prompting, denoted as \evalperfrandom and \evalperfslow.

% \textit{Direct prompting.} To highlight the importance of asking the language model to generate pc-constraints instead of directly generating the input itself (or an input generator), we also evaluate \tool against a straightforward stress-test generation approach: we instruct the language model to synthesize a program that generates performance-exercising inputs directly. 
\textit{Direct Prompting.} \citet{du2024mercury}, \citet{peng2025coffecodeefficiencybenchmark}, and \citet{huang-neurips24-effibench} respectively prompts an \llm to produce the test case generator to generate massive test cases with different input sizes, data distribution, and edge cases~\footnote{At the time we run the experiments, the prompts and scripts for test case generation have not been available, so we try to adopt a similar idea to our dataset.}.
To understand how well directly prompting an \llm to synthesize an input generator without few-shot CoT prompting and scale controlling can perform, we design \directprompting for comparison.
\directprompting directly prompts the \llm to produce a generator script to identify and implement input patterns that can stress the solutions to the given problem statement the most.

For the prompting-based techniques, we generate 20 tests per problem to ensure fairness, following the setting of prior study~\cite{peng2025coffecodeefficiencybenchmark}.



\para{Metrics.}
% PIE~\cite{shypula-iclr24}, EffiBench~\cite{huang-neurips24-effibench} and EvalPerf~\cite{liu-colm24}
Prior works respectively rely on CPU simulators like Gem5~\cite{binkert2011gem5} (PIE~\cite{shypula-iclr24}), physical execution time (EffiBench~\cite{huang-neurips24-effibench}, Mercury~\cite{du2024mercury}), and hardware performance counters~\cite{wiki:Hardware_performance_counter} (EvalPerf~\cite{liu-colm24}, COFFE~\cite{peng2025coffecodeefficiencybenchmark}).
Gem5 is known to be stable, but the overhead is significant and the CPU simulator does not necessarily reflect the physical performance.
% Physical execution time is most susceptible to the noise from environment, and the results should be interpreted with caution.
While physical running time offers intuitive measure, it is susceptible to interfere from transient system effects--such as background processes, scheduling variability, and I/O fluctuations--which can obscure true computational cost.
In contrast, hardware performance counters provides a more stable, low-noise, and platform-agnostic metric.
It records the number of executed instructions of a program execution using the Linux \texttt{perf} tool~\cite{de2010new}.
It incurs low overhead and it's highly reproducible.
Moreover, \citet{peng2025coffecodeefficiencybenchmark} demonstrates that it is 1000X more stable than physical execution time and it's linearly correlated with execution time with Pearson correlation coefficient of 0.96 \textasciitilde 1.0.
% But it's not necessarily linearly related to physical performance.
% All three metrics were used in our evaluation (for different experiments).
% To measure performance, we consider both physical execution time and the instruction count based on hardware performance counters~\cite{wiki:Hardware_performance_counter}.
% Instruction counts are collected using the Linux \texttt{perf} tool~\cite{de2010new}.
% While physical running time offers intuitive measure, it is susceptible to interfere from transient system effects--such as background processes, scheduling variability, and I/O fluctuations--which can obscure true computational cost.
% Therefore, timing-based results should be interpreted with caution.
% In contrast, instruction count provides a more stable, low-noise, and platform-agnostic metric. Prior work has shown that instruction count correlates strongly with execution characteristics indicative of performance bottlenecks~\cite{curtsinger-sosp15,delimitrou-asplos14,iorgulescu-atc18,liu-colm24,zhang-eurosys13}.
Therefore, we use \#instructions as our main evaluation metric (meanwhile we attach the corresponding physical execution time results in appendix).


For each program, we execute all tests generated by each technique and record the \#instructions and physical runtime.
For a fair comparison, we select the slowest test inputs (top-10, top-5, top-3, top-1) per solution for each technique to compare.
We also compare \tool with the baseline techniques in terms of number of programs \tool can or cannot outperform the baseline techniques.
We provide a fine-grained pairwise comparison between \tool tests and baseline tests to show the distribution of normalized ratio of \tool tests v.s. baseline tests.

% We are aware of a more precise time measurement using GEM5 emulators



% \para{Language models.} We use XX model with YY setting. We use TT model with WW setting. 

% \para{Language models.} For all prompting baseline experiments and steps, we use the OpenAI GPT-4o (gpt-4o-2024-08-06) with a temperature of 0.8 and max\_length of 4096.

\para{Implementation.} We run experiments on six x86-64 machines equipped with a 24-core Intel Xeon Gold 6126 CPU with 192GB of RAM.
Each machine runs Ubuntu 20.04 LTS (kernel version 5.4.0).
We use the OpenAI GPT-4o (gpt-4o-2024-08-06) with a temperature of 0.8 and max\_length of 4,096.

\begin{table*}[!t]

    \centering
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1}
    \small

  \caption{Comparison between \tool and baseline techniques. Average \#instructions ($\times 10^9$) and relative slowdown compared with default tests across all tested programs running top-$k$, $k={10, 5, 3, 1}$ slowest inputs.}
  \label{tab:instruction-count}


\begin{tabular}{lllll}
\toprule
\# of slowest inputs & Top-10 & Top-5 & Top-3 & Top-1 \\ \midrule
\rowcolor[gray]{0.95}\multicolumn{5}{c}{Number of instructions ($\times 10^9$)} \\
wedge & \textbf{1.03$\pm$0.00} & \textbf{1.15$\pm$0.00} & \textbf{1.24$\pm$0.00} & \textbf{1.49$\pm$0.00} \\
direct-prompt & 0.50$\pm$0.00 ($\textcolor{red}{\downarrow}2.1\times$) & 0.61$\pm$0.00 ($\textcolor{red}{\downarrow}1.9\times$) & 0.69$\pm$0.00 ($\textcolor{red}{\downarrow}1.8\times$) & 0.87$\pm$0.00 ($\textcolor{red}{\downarrow}1.7\times$) \\
evalperf-slow & 0.40$\pm$0.00 ($\textcolor{red}{\downarrow}2.6\times$) & 0.49$\pm$0.00 ($\textcolor{red}{\downarrow}2.3\times$) & 0.55$\pm$0.00 ($\textcolor{red}{\downarrow}2.3\times$) & 0.61$\pm$0.00 ($\textcolor{red}{\downarrow}2.5\times$) \\
evalperf-rand & 0.43$\pm$0.00 ($\textcolor{red}{\downarrow}2.4\times$) & 0.52$\pm$0.00 ($\textcolor{red}{\downarrow}2.2\times$) & 0.57$\pm$0.00 ($\textcolor{red}{\downarrow}2.2\times$) & 0.64$\pm$0.00 ($\textcolor{red}{\downarrow}2.3\times$) \\
\midrule
\rowcolor[gray]{0.95}\multicolumn{5}{c}{Running time (ms)} \\
wedge & \textbf{250$\pm$0.2} & \textbf{271$\pm$0.2} & \textbf{286$\pm$0.2} & \textbf{334$\pm$0.2} \\
direct-prompt & 170$\pm$0.1 ($\textcolor{red}{\downarrow}1.5\times$) & 194$\pm$0.1 ($\textcolor{red}{\downarrow}1.4\times$) & 213$\pm$0.1 ($\textcolor{red}{\downarrow}1.3\times$) & 260$\pm$0.1 ($\textcolor{red}{\downarrow}1.3\times$) \\
evalperf-slow & 121$\pm$0.1 ($\textcolor{red}{\downarrow}2.1\times$) & 143$\pm$0.1 ($\textcolor{red}{\downarrow}1.9\times$) & 157$\pm$0.2 ($\textcolor{red}{\downarrow}1.8\times$) & 172$\pm$0.2 ($\textcolor{red}{\downarrow}1.9\times$) \\
evalperf-rand & 125$\pm$0.1 ($\textcolor{red}{\downarrow}2.0\times$) & 148$\pm$0.1 ($\textcolor{red}{\downarrow}1.8\times$) & 160$\pm$0.2 ($\textcolor{red}{\downarrow}1.8\times$) & 177$\pm$0.2 ($\textcolor{red}{\downarrow}1.9\times$) \\
\bottomrule
\end{tabular}


% \begin{tabular}{lllll}\toprule \# of slowest inputs & Top-10 & Top-5 & Top-3 & Top-1 \\ \midrule
% \rowcolor[gray]{0.95} \multicolumn{4}{c}{Relative slowdown compared with default tests} \\
%  \tool & \textbf{4.61} & \textbf{4.30} & \textbf{4.17} & \textbf{3.96}  \\ \evalperfrandom & 2.44 & 2.97 & 3.22 & 3.38  \\ \evalperfslow & 2.44 & 2.95 & 3.19 & 3.31  \\ \directprompting & 3.73 & 3.86 & 3.97 & 4.34  \\ \midrule
% \rowcolor[gray]{0.95} \multicolumn{4}{c}{Number of instructions ($\times 10^8$)} \\
%  \tool & \textbf{3.85} & \textbf{3.93} & \textbf{3.99} & \textbf{4.06}  \\ \evalperfrandom & 2.04 & 2.71 & 3.08 & 3.47  \\ \evalperfslow & 2.03 & 2.70 & 3.05 & 3.39  \\ \directprompting & 3.12 & 3.53 & 3.80 & 4.45  \\ \bottomrule
% \end{tabular} 

% \begin{tabular}{lllll}\toprule \# of slowest inputs & Top-10 & Top-5 & Top-3 & Top-1 \\ \midrule
% \rowcolor[gray]{0.95} \multicolumn{4}{c}{Relative slowdown compared with default tests} \\
%  \tool & \textbf{6.58} & \textbf{6.34} & \textbf{6.31} & \textbf{6.64}  \\ \evalperfrandom & 3.32 & 3.78 & 4.04 & 4.16  \\ \evalperfslow & 3.26 & 3.73 & 3.96 & 4.04  \\ \directprompting & 4.53 & 4.63 & 4.78 & 5.39  \\ \midrule
% \rowcolor[gray]{0.95} \multicolumn{4}{c}{Number of instructions ($\times 10^8$)} \\
%  \tool & \textbf{5.56} & \textbf{5.89} & \textbf{6.13} & \textbf{6.93}  \\ \evalperfrandom & 2.80 & 3.51 & 3.92 & 4.34  \\ \evalperfslow & 2.76 & 3.46 & 3.84 & 4.21  \\ \directprompting & 3.83 & 4.29 & 4.64 & 5.63  \\ \bottomrule
% \end{tabular}

% \begin{tabular}{lllll}\toprule \# of slowest inputs & Top-10 & Top-5 & Top-3 & Top-1 \\ \midrule
% \rowcolor[gray]{0.95} \multicolumn{4}{c}{Relative slowdown compared with default tests} \\
%  \tool & \textbf{4.61} & \textbf{4.30} & \textbf{4.17} & \textbf{3.96}  \\ \evalperfrandom & 2.44 & 2.97 & 3.22 & 3.38  \\ \evalperfslow & 2.44 & 2.95 & 3.19 & 3.31  \\ \directprompting & 3.73 & 3.86 & 3.97 & 4.34  \\ \midrule
% \rowcolor[gray]{0.95} \multicolumn{4}{c}{Number of instructions ($\times 10^8$)} \\
%  \tool & \textbf{3.85} & \textbf{3.93} & \textbf{3.99} & \textbf{4.06}  \\ \evalperfrandom & 2.04 & 2.71 & 3.08 & 3.47  \\ \evalperfslow & 2.03 & 2.70 & 3.05 & 3.39  \\ \directprompting & 3.12 & 3.53 & 3.80 & 4.45  \\ \bottomrule
% \end{tabular}

% \begin{tabular}{lllll}\toprule \# of slowest inputs & Top-10 & Top-5 & Top-3 & Top-1 \\ \midrule
% \rowcolor[gray]{0.95} \multicolumn{5}{c}{Relative slowdown compared with default tests} \\
%  \tool & \textbf{7.92} & \textbf{8.15} & \textbf{8.56} & \textbf{10.36}  \\ \evalperfrandom & 4.01 & 4.47 & 4.72 & 4.80  \\ \evalperfslow & 3.71 & 4.15 & 4.41 & 4.49  \\ \directprompting & 4.58 & 4.69 & 4.86 & 5.51  \\ \midrule
% \rowcolor[gray]{0.95} \multicolumn{5}{c}{Number of instructions ($\times 10^8$)} \\
%  \tool & \textbf{6.55} & \textbf{7.41} & \textbf{8.15} & \textbf{10.60}  \\ \evalperfrandom & 3.32 & 4.06 & 4.49 & 4.92  \\ \evalperfslow & 3.07 & 3.77 & 4.20 & 4.59  \\ \directprompting & 3.79 & 4.26 & 4.63 & 5.64  \\ \bottomrule
% \end{tabular}



\end{table*}

\subsection{Main Result}
\label{sec:quantitative_results}
As Table~\ref{tab:instruction-count} shows, \tool tests can lead to 4.44x $\sim$ 4.86x slowdown compared with \codecontest tests (including public tests and private tests from \codeforces dataset and generated tests generatedy by \alphacode paper authors~\cite{li-science22}) in terms of \#instructions.
% 
We also calculate the number of programs where \tool can or cannot outperform \evalperfslow/\evalperfrandom/\directprompting, as shown in Table~\ref{tab:histogram-bins} and Figure~\ref{fig:histogram_head_to_head}.
\tool substantially generate slower tests on more programs than all baseline techniques.
Specifically, \tool performs better than \evalperfslow and \evalperfrandom on up to 93.5\% solutions, and better than \directprompting on up to 89.0\% solutions.
% 
% Overall, on xx\% (top-1 inputs) programs \tool can generate the slowest tests .
% 


% \subsection{Qualitative Analysis}
% \label{sec:qualitative_results}
We manually inspect several cases where \tool tests significantly outperform baseline tests and make the following observations.
One notable example is \codeforces Problem 633A (Figure~\ref{fig:motivating}), where \tool tests significantly outperform \evalperfrandom, \evalperfslow, \directprompting tests.
% We examined the input generators synthesized by \evalperfslow, \evalperfrandom, \directprompting, as shown in \ref{lst:p633a-evalperfslow}, \ref{lst:p633a-evalperfrandom}, and \ref{lst:p633a-directprompting} respectively.
The input generators synthesized by the baselines are shown in Listing~\ref{lst:p633a-evalperfrandom}, Listing~\ref{lst:p633a-evalperfslow}, and Listing~\ref{lst:p633a-directprompting}.
It turns out that \evalperfslow generator will only generate the inputs near the upper bounds, \ie (99, 100, 10000), without even utilizing the \codeIn{scale} parameter.
\evalperfrandom generates random a and b within the range [1, 100] and a large c (determined by \codeIn{scale}) as the input.
\directprompting composes a series of concrete test cases rather than synthesizing a pattern-based generator.
While it attempts to implicitly reason about how to stress the solutions by including diverse patterns, there is little guarantee that these patterns can trigger performance bottlenecks.

% \begin{lstinputlisting}
% [language=Python, numbers=none, caption={\evalperfslow synthesized generator for Problem 633A}, label={lst:p633a-evalperfslow}, escapechar=!<>, lineskip=-1pt]
% {listings/633_A_evalperf_slow_gen.py}
% \end{lstinputlisting}

% \begin{lstinputlisting}
% [language=Python, numbers=none, caption={\evalperfrandom synthesized generator for Problem 633A}, label={lst:p633a-evalperfrandom}, escapechar=!<>, lineskip=-1pt]
% {listings/633_A_evalperf_random_gen.py}
% \end{lstinputlisting}

In contrast, \tool relies on fuzzing with constraint-aware mutators to efficently search for a diverse set of constraint-satisfying inputs.
Listing~\ref{lst:p633a-wedge} shows a constraint-aware mutator for Problem 633A.
The mutator will mutate a previous input (seed input) to produce the next input (mutated input).
The while loop will search the input space of (\codeIn{a, b, c}) and ensure they conform to the constraints \codeIn{not abs (a - b) > 5 or c \% a == 0 or c \% b == 0}, \ie \codeIn{abs (a - b) <= 5 and c \% a != 0 and c \% b != 0} (already satisfying the first two out of three constraints in Listing~\ref{lst:p633a-constraint-checker}).
As a result, the average \#instructions (using top-5 inputs) of \tool substantially outperforms the baseline techniques by 4.16$\times$, 7.22$\times$, and 1.70$\times$ on Problem 633A, respectively.
   
% 




\begin{figure*}[!t]

\centering

\subfloat[\tool vs.\evalperfslow]{
        \includegraphics[width=0.24\linewidth]{figures/areachart_wedge_vs_evalperf-slow_top10inputs.pdf}
        \label{subfig:areachart_wedge_vs_evalperf-slow_top10inputs}
    }
\subfloat[\tool vs.\evalperfrandom]{
        \includegraphics[width=0.24\linewidth]{figures/areachart_wedge_vs_evalperf-rand_top10inputs.pdf}
        \label{subfig:areachart_wedge_vs_evalperf-rand_top10inputs}
    }
\subfloat[\tool vs.\directprompting]{
        \includegraphics[width=0.24\linewidth]{figures/areachart_wedge_vs_direct-prompt_top10inputs.pdf}
        \label{subfig:areachart_wedge_vs_direct-prompt_top10inputs}
    }
    
\caption{
\end{figure*}




\begin{figure*}[!t]

\centering

\captionsetup[subfigure]{labelformat=empty,font=small}

\subfloat[vs.\evalperfslow (top-10)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-slow_top10inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-slow_top10inputs}
    }
\subfloat[vs.\evalperfslow (top-5)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-slow_top5inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-slow_top5inputs}
    }
\subfloat[vs.\evalperfslow (top-3)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-slow_top3inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-slow_top3inputs}
    }
\subfloat[vs.\evalperfslow (top-1)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-slow_top1inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-slow_top1inputs}
    }

\subfloat[vs.\evalperfrandom (top-10)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-rand_top10inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-rand_top10inputs}
    }
\subfloat[vs.\evalperfrandom (top-5)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-rand_top5inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-rand_top5inputs}
    }
\subfloat[vs.\evalperfrandom (top-3)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-rand_top3inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-rand_top3inputs}
    }
\subfloat[vs.\evalperfrandom (top-1)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_evalperf-rand_top1inputs.pdf}
        \label{subfig:histogram_wedge_vs_evalperf-rand_top1inputs}
    }

\subfloat[vs.\directprompting (top-10)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_direct-prompt_top10inputs.pdf}
        \label{subfig:histogram_wedge_vs_direct-prompt_top10inputs}
    }
\subfloat[vs.\directprompting (top-5)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_direct-prompt_top5inputs.pdf}
        \label{subfig:histogram_wedge_vs_direct-prompt_top5inputs}
    }
\subfloat[vs.\directprompting (top-3)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_direct-prompt_top3inputs.pdf}
        \label{subfig:histogram_wedge_vs_direct-prompt_top3inputs}
    }
\subfloat[vs.\directprompting (top-1)]{
        \includegraphics[width=0.24\linewidth]{figures/histogram_wedge_vs_direct-prompt_top1inputs.pdf}
        \label{subfig:histogram_wedge_vs_direct-prompt_top1inputs}
    }

\caption{Comparisons between \tool (\textcolor{CustomOrange}{\ding{110}}) and the other baselines (\textcolor{CustomPurple}{\ding{110}}). The bars represent the number of programs where one of the tools incurs a larger instruction count when running over the top-$k$ ($k=\{1,3,5,10\}$) slowest inputs generated by our tool.}
\label{fig:histogram_head_to_head}

\end{figure*}

% Figure~\ref{fig:histogram_head_to_head} shows


\subsection{Ablations}
\label{sec:ablations}
% We ablate each design choice, i.e., (1) constraint-aware mutator, (2) constraint-instrumented fuzz driver, and the combination of (1) and (2), to investigate their contribution to \tool.
% To further demonstrate the contribution of a constraint-aware mutator, we compare a constraint-aware mutator against a strong \llm-generated baseline that only leverages the problem statement.

We ablate each design choice, \ie (1) involving \textbf{performance-characterizing constraints} in mutator generation, (2) instrumenting the original program with \textbf{constraint checker} branches, to investigate their contribution to \tool.
For (1), we use a constraint-agnostic mutator for comparison.
For (2), we use the original program for comparison.
We also include plain \afl without the above designs as a baseline.
The constraint-aware mutator and constraint-agnostic mutator are generated by prompting with and without the performance constraints.
% The default mutator is the AFL++ default mutator, not aware of any validity/performance constraints.
The constraint-agnostic mutator is generated by prompting with the problem statement only.
The constraint-aware mutator is generated by prompting both the problem statement and performance constraints.
 
% impact of each key design choice in \tool, we evaluate three ablated fuzzing-based techniques to compare with \tool:
% \begin{itemize}
%     \item \textbf{\tool}. Use the \textbf{constraint-aware} mutator + use the \textbf{instrumented program} (w/ constraint) as the fuzz driver. (afl++ + PC-constraint-aware mutator)
%     % \item \textbf{\wedgenoinstrument}. Use the \textbf{constraint-aware} mutator + use the \textbf{original program} (w/o constraint) as the fuzz driver. (afl++ + PC-constraint-aware mutator)
%     \item \textbf{\wedgenoconstraint}. Use the \textbf{constraint-agnostic} mutator + use the \textbf{original program} (w/o constraint) as the fuzz driver. (afl++ + validity)
%     \item \textbf{\wedgenomutator}. Use the \textbf{default mutator} + use the \textbf{original program} (w/o constraint) as the fuzz driver. (afl++)
% \end{itemize}
\begin{comment}
\vspace{5mm}
\noindent
\begin{wraptable}{r}{0.6\textwidth} 
\begin{minipage}{\linewidth}
% \begin{table}[!t]

    \centering
    \setlength{\tabcolsep}{8pt}
    \renewcommand{\arraystretch}{1}
    \small

  \caption{Comparison between \tool and ablated versions. Average \#instructions ($\times 10^8$) and relative slowdown compared with default tests across all tested programs running top-$k$, $k={10, 5, 3}$ slowest inputs.}
  \label{tab:ablation}

\begin{tabular}{lllll}\toprule \# of slowest inputs & Top-10 & Top-5 & Top-3 & Top-1 \\ \midrule
\rowcolor[gray]{0.95} \multicolumn{5}{c}{Relative slowdown compared with default tests} \\
 \wedgenomutator & 1.53 & 1.94 & 2.46 & 3.59  \\ \wedgenoconstraint & 242.16 & 365.37 & 424.16 & 423.97  \\ \wedgenoinstrument & 391.93 & 472.51 & 561.46 & 703.19  \\ \tool & \textbf{513.21} & \textbf{594.58} & \textbf{654.49} & \textbf{803.62}  \\ \midrule
\rowcolor[gray]{0.95} \multicolumn{5}{c}{Number of instructions ($\times 10^8$)} \\
 \wedgenomutator & 0.68 & 0.77 & 0.81 & 0.91  \\ \wedgenoconstraint & 3.00 & 4.05 & 4.69 & 5.07  \\ \wedgenoinstrument & 5.29 & 6.12 & 6.98 & 8.91  \\ \tool & \textbf{6.58} & \textbf{7.45} & \textbf{8.19} & \textbf{10.66}  \\ \bottomrule
\end{tabular}

\begin{tabular}{c|c|c}\toprule
Setting & mutator & fuzz driver \\ \midrule
\wedgenomutator & AFL++ default mutator & $\mathcal{P}$ \\
\wedgenoconstraint & constraint-agnostic mutator & $\mathcal{P}$ \\ 
\wedgenoinstrument & constraint-aware mutator & $\mathcal{P}$ \\ 
\tool & constraint-aware mutator & $\mathcal{P'}$ \\ 
\bottomrule
\end{tabular}
\end{minipage}
\end{wraptable}
\end{comment}

% \begin{wraptable}{r}{0.95\linewidth}
\begin{table}
\centering
\small
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.1}
\caption{Comparison between \tool and ablated versions. We report relative slowdown compared with default tests and average instruction count ($\times 10^8$) across all tested programs using the top-$k$ slowest inputs ($k=10, 5, 3, 1$).}
\label{tab:ablation}

% \begin{tabular}{lllll}\toprule \# of slowest inputs & Top-10 & Top-5 & Top-3 & Top-1 \\ \midrule
% \rowcolor[gray]{0.95} \multicolumn{5}{c}{Relative slowdown compared with default tests} \\
%  \wedgenomutator & 1.53 & 1.94 & 2.46 & 3.59  \\ \wedgedefault & 8.50 & 14.80 & 22.34 & 50.19  \\ \wedgenoconstraint & 242.16 & 365.37 & 424.16 & 423.97  \\ \wedgecustom & 342.98 & 442.40 & 458.79 & 457.04  \\ \wedgenoinstrument & 391.93 & 472.51 & 561.46 & 703.19  \\ \tool & \textbf{513.21} & \textbf{594.58} & \textbf{654.49} & \textbf{803.62}  \\ \midrule
% \rowcolor[gray]{0.95} \multicolumn{5}{c}{Number of instructions ($\times 10^8$)} \\
%  \wedgenomutator & 0.68 & 0.77 & 0.81 & 0.91  \\ \wedgedefault & 0.79 & 0.96 & 1.13 & 1.70  \\ \wedgenoconstraint & 3.00 & 4.05 & 4.69 & 5.07  \\ \wedgecustom & 3.95 & 4.89 & 5.18 & 5.64  \\ \wedgenoinstrument & 5.29 & 6.12 & 6.98 & 8.91  \\ \tool & \textbf{6.58} & \textbf{7.45} & \textbf{8.19} & \textbf{10.66}  \\ \bottomrule
% \end{tabular}

\begin{tabular}{lllll}\toprule \# of slowest inputs & Top-10 & Top-5 & Top-3 & Top-1 \\ \midrule
\rowcolor[gray]{0.95} \multicolumn{5}{c}{Relative slowdown compared with default tests} \\
 \wedgenoconstraint & 242.16 & 365.37 & 424.16 & 423.97  \\ \wedgecustom & 342.98 & 442.40 & 458.79 & 457.04  \\ \wedgenoinstrument & 391.93 & 472.51 & 561.46 & 703.19  \\ \toolfull & \textbf{513.21} & \textbf{594.58} & \textbf{654.49} & \textbf{803.62}  \\ \midrule
\rowcolor[gray]{0.95} \multicolumn{5}{c}{Number of instructions ($\times 10^8$)} \\
 \wedgenoconstraint & 3.00 & 4.05 & 4.69 & 5.07  \\ \wedgecustom & 3.95 & 4.89 & 5.18 & 5.64  \\ \wedgenoinstrument & 5.29 & 6.12 & 6.98 & 8.91  \\ \toolfull & \textbf{6.58} & \textbf{7.45} & \textbf{8.19} & \textbf{10.66}  \\ \bottomrule
\end{tabular}

\end{table}

Table~\ref{tab:ablation} shows the performance of \tool and ablated versions.
\tool tests (using top-10 inputs) are on average 63.03\% and 62.34\% slower (in terms of relative slowdown and \#instructions) than \wedgenoinstrument.
The results show using instrumented programs (programs with constraint checkers inserted) can provide guidance to fuzzing, thus generating slower tests compared with not inserting the checkers.
Similarly, \wedgenoinstrument tests are on average 155.17\% and 156.99\% slower than \wedgenoconstraint.
On 63.02\% solutions \wedgenoinstrument tests are slower (with a significance value of 0.05, according to Mann-Whitney test~\cite{mcknight2010mann}).
This underscores the importance of the performance-constraint-aware mutator.



% Out of curiosity, we also evaluate using AFL++ default mutator.
% It turns out \wedgenomutator performs worse than \wedgenoconstraint by 29.03\% on average (in terms of slowdown and \#instructions), indicating even validity-aware mutators are better than the default mutators.
% The validation result shows that the validity rate of \wedgenoconstraint is 58.05\% higher than \wedgenomutator.
% 
% 

\subsection{Effect of Constraints.}
\para{Discrimination of performance-characterizing constraints.}
To investigate whether and how \tool generated performance-characterizing constraints can classify inputs, we select a set of 813 solution programs where both constraint-satisfying inputs and constraint-violating inputs exist.
We compare the average \#instructions of both sets on each solution.
Constraint-satisfying inputs are on average 51.46$\times$ slower than constraint-violating inputs.
We conduct a Mann-Whitney test~\cite{mcknight2010mann}, and constraint-satisfying inputs are significantly slower (with a significance value p < 0.05) than constraint-violating inputs on 93.73\% solution programs.
It demonstrates the performance-characterizing constraints generated by \tool are discriminative across most programs.

\para{Impact of constraints in guiding fuzzing.}
To better understand the impact of guidance of constraints (including mutator and fuzz driver instrumentation), we calculate the ratio of constraint-satisfying inputs (out of valid inputs) per strategy.
The result shows involving performance-constraints and constraint-checking branches contribute positively to the ratio of constraint-satisfying inputs.
Specifically, the ratios of constraint-satisfying inputs among generated inputs of \wedgenoconstraint, \wedgenoinstrument, and \tool are 49.11\%, 77.62\% and 80.48\% respectively.

\subsection{Utility of \bench Tests}
\label{sec:tests-utility}

% \para{Utility in improving code optimization approaches based on execution feedback}.
\para{Code optimization with execution feedback.}
% \cite{huang-neurips24} proposed \effilearner, utilizing execution overhead profiles to improve the efficiency of \llm-generated code. However, the approach utilizes public test cases to guide code efficiency optimization, while public tests might be not stressing enough to reveal inefficiencies of code. Driven by curiosity, we aim to leverage the stressing tests generated by \tool to improve the code optimization performance.
Execution feedback has been shown to be helpful in \llm-based code editing~\cite{chunqiu-issta24,peng2024perfcodegen,huang-neurips24}.
Execution feedback relies on high-quality tests.
We use \bench tests to provide execution feedback for \llm-based code performance optimization to show the usefulness of our tests.
\cite{huang-neurips24} proposed \effilearner, utilizing execution feedback (profiling information) to improve the efficiency of \llm-generated code. 
However, the approach utilizes a limited set of public tests which might not be stressing enough to reveal inefficiencies of code.
Therefore, we replace the public tests with our tests to investigate how stressing tests can help improve the code optimization workflow.
% % To be clear, we select \placeholder slow solutions of \placeholder problems from \bench, execute the default tests and our generated tests, collect the profiling feedback correspondingly, and prompt the model to produce edited programs. Then we profile the edited programs to collect the statistics following settings of \effilearner, and compare the performance in terms of optimization.
Specifically, we select 280 slow Python solutions from 56 problems (filtering process detailed in Appendix~\ref{sec:utility_filtering}), execute the default tests and our generated tests, collect the profiling feedback respectively, and prompt the model to produce edited programs. Then we evaluate the edited programs following settings of \effilearner~\cite{huang-neurips24}, and compare the performance.
For each solution, we apply three different prompting strategies for optimization: prompting without profiling information, prompting with profiling information running \codecontest public tests, and prompting with profiling information running \tool tests, denoted as \textbf{No\_Profile}, \textbf{Public\_Profile}, and \textbf{Wedge\_Profile} respectively.
% For models, we include the most powerful business model and open-source model at the moment this paper is written, namely OpenAI GPT-4o and DeepSeek V3. For configurations \eg, temperature, max\_length, we reused the setting in the main experiment.
% Following the workflow of \effilearner, we profile the solutions written by users and prompt the model with the feedback information to optimize the solutions, then we evaluate the correctness and efficiency of the optimized solutions. Note that we only evaluate the efficiency of the correct optimized solutions, and when we compare two strategies, we evaluate on the overlapping set of solutions where both strategies produce the correct optimized solutions. We include three metrics from \effilearner work~\cite{huang-neurips24}, namely ET (Execution Time), MU (Maximum Memory Usage), TU (Total Memory Usage), and one additional metric ICT (Instruction Count). We didn't include the other three metrics (the corresponding normalized ones) from \effilearner work as we don't have the "canonical" solution in our dataset.
For models, we include OpenAI GPT-4o and DeepSeek V3. We reused the same prompting settings (temperature, max\_length, \etc) in the main experiment. We include three metrics from \effilearner work~\cite{huang-neurips24}, namely Execution Time, Maximum Memory Usage, Total Memory Usage, and one additional metric Instruction Count.
We didn't include the other three metrics (the corresponding normalized ones) from \effilearner work as we don't have the ``canonical'' solution in our dataset.

As shown in Table~\ref{tab:effilearner-experiment}, by using stress tests from \tool, both GPT-4o and DeepSeek-V3 can lead to more performance improvement compared with not using profiling information or using profiling information from public tests in most metrics, surpassing the second best by 3.32-9.42pp (percentage points) except one metric. In addition, even prompting with profiling information from just five public inputs can substantially outperform prompting with no profiling information, which confirms the insight of \cite{huang-neurips24}, while slow stressing tests can even enlarge the improvement.

% \begin{table*}[!t]

%     \centering
%     \setlength{\tabcolsep}{4pt}
%     \renewcommand{\arraystretch}{1}
%     \small

%   \caption{EffiLearner Experiment}
%   \label{tab:effilearner-experiment}
% \begin{tabular}{rlrrrr}
% \toprule
% \textbf{Model} & \textbf{Test Input Set} & \multicolumn{1}{l}{\textbf{Execution Time (s)}} & \multicolumn{1}{l}{\textbf{Total Memory Usage (Mb * s)}} & \multicolumn{1}{l}{\textbf{Max Memory Usage (Mb)}} & \multicolumn{1}{l}{\textbf{Execution Time (\#inst)}} \\ \midrule
% \multirow{3}{*}{GPT-4o} & \noprofile & 15.66\% & 21.70\% & 2.78\% & 31.39\% \\
%  & \publicfiveprofile & 22.57\% & 27.78\% & \textbf{11.89\%} & 39.89\% \\
%  & \wedgeprofile & \textbf{26.47\%} & \textbf{35.10\%} & 11.82\% & \textbf{49.31\%} \\ \midrule
% \multirow{3}{*}{DeepSeek-V3} & \noprofile & 6.77\% & 12.49\% & 2.30\% & 20.48\% \\
%  & \publicfiveprofile & 12.29\% & 20.43\% & 1.93\% & 35.01\% \\
%  & \wedgeprofile & \textbf{18.99\%} & \textbf{23.75\%} & \textbf{9.21\%} & \textbf{40.26\%} \\ \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}[!t]
%     \centering
%     \setlength{\tabcolsep}{4pt}
%     \renewcommand{\arraystretch}{1}
%     \small

%     \caption{EffiLearner Experiment}
%     \label{tab:effilearner-experiment}
%     \begin{tabular}{rlr|r r|r}
%         \toprule
%         \textbf{Model} & \textbf{Test Input Set} & \textbf{Execution Time (s)} & \multicolumn{2}{c|}{\textbf{Memory Usage}} & \textbf{Execution Time (\#inst)} \\
%         \cmidrule{4-5}
%         & & & \textbf{Total (Mb * s)} & \textbf{Max (Mb)} &  \\
%         \midrule
%         \multirow{3}{*}{GPT-4o} 
%         & no\_profile & 15.66\% & 21.70\% & 2.78\% & 31.39\% \\
%         & public\_profile & 22.57\% & 27.78\% & \textbf{11.89\%} & 39.89\% \\
%         & wedge\_profile & \textbf{26.47\%} & \textbf{35.10\%} & 11.82\% & \textbf{49.31\%} \\ 
%         \midrule
%         \multirow{3}{*}{DeepSeek-V3} 
%         & no\_profile & 6.77\% & 12.49\% & 2.30\% & 20.48\% \\
%         & public\_profile & 12.29\% & 20.43\% & 1.93\% & 35.01\% \\
%         & wedge\_profile & \textbf{18.99\%} & \textbf{23.75\%} & \textbf{9.21\%} & \textbf{40.26\%} \\ 
%         \bottomrule
%     \end{tabular}
% \end{table*}

\begin{table*}[!t]
    \centering
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1}
    \small

    \caption{EffiLearner Experiment}
    \label{tab:effilearner-experiment}
    \begin{tabular}{rlr|r|r|r}
        \toprule
        \textbf{Model} & \textbf{Test Input Set} & \makecell{\textbf{Execution} \\ \textbf{Time (s)}} &
        \makecell{\textbf{Total Memory} \\ \textbf{Usage (Mb * s)}} &
        \makecell{\textbf{Max Memory} \\ \textbf{Usage (Mb)}} &
        \makecell{\textbf{Execution} \\ \textbf{Time (\#inst)}} \\
        \midrule
        \multirow{3}{*}{GPT-4o} 
          & no\_profile     & 15.66\%              & 21.70\%         & 2.78\%           & 31.39\% \\
          & public\_profile & 22.57\%              & 27.78\%         & \textbf{11.89\%} & 39.89\% \\
          & wedge\_profile  & \textbf{26.47\%}     & \textbf{35.10\%}& 11.82\%          & \textbf{49.31\%} \\ 
        \midrule
        \multirow{3}{*}{DeepSeek-V3} 
          & no\_profile     & 6.77\%               & 12.49\%         & 2.30\%           & 20.48\% \\
          & public\_profile & 12.29\%              & 20.43\%         & 1.93\%           & 35.01\% \\
          & wedge\_profile  & \textbf{18.99\%}     & \textbf{23.75\%}& \textbf{9.21\%}  & \textbf{40.26\%} \\ 
        \bottomrule
    \end{tabular}
\end{table*}





\begin{table*}[!t]

    \centering
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1}
    \small

  \caption{Pie Experiment}
  \label{tab:pie-experiment}
\begin{tabular}{rlrrrr}
\toprule
\textbf{Model} & \textbf{Test Input Set} & \multicolumn{1}{l}{\textbf{Speedup (\#inst)}} & \multicolumn{1}{l}{\textbf{Speedup (time)}} & \multicolumn{1}{l}{\textbf{\%Opt (\#inst)}} & \multicolumn{1}{l}{\textbf{\%Opt (time)}} \\ \midrule
\multirow{3}{*}{\piehq} & \defaultall & 1.32 & 0.93 & 6.03\% & 16.58\% \\
 & \defaultslowfive & 1.30 & 0.94 & 5.53\% & 18.09\% \\
 & \wedgeslowfive & \textbf{1.62} & \textbf{1.18} & \textbf{12.06\%} & \textbf{26.63\%} \\ \midrule
\multirow{3}{*}{\piecond} & \defaultall & 1.98 & 1.13 & 16.23\% & 29.22\% \\
 & \defaultslowfive & 1.85 & 1.13 & 15.58\% & 27.92\% \\
 & \wedgeslowfive & \textbf{1.99} & \textbf{1.29} & \textbf{18.83\%} & \textbf{41.56\%} \\ \midrule
\multirow{3}{*}{\pieuncond} & \defaultall & 1.21 & 1.32 & 4.35\% & 56.52\% \\
 & \defaultslowfive & 1.21 & 1.32 & 4.35\% & 56.52\% \\
 & \wedgeslowfive & \textbf{3.01} & \textbf{1.38} & \textbf{30.43\%} & \textbf{60.87\%} \\ \bottomrule
\end{tabular}
\end{table*}

% \subsubsection{Evaluating Performance Improvement of Code Optimization Model with Different Tests}
% LLMs have been extensively used in code optimization in the recent works~\cite{shypula-iclr24,gao-icse24,cummins-arxiv24}, however, they rely on a limited set of tests that were created to evaluate correctness when evaluating performance improvement. While those correctness tests might not be stressing enough to reveal the difference between a slow program and a fast, optimized program. To investigate how stress tests generated by \tool can help show the performance improvement of code optimization models, we adapt the state-of-the-art code optimization technique~\cite{shypula-iclr24} to our framework. 
% Specifically, we picked the most powerful models finetuned by \cite{shypula-iclr24} authors, 13b CodeLlama model finetuned on HQ + self-play augmented data (denoted as \piehq) and 13b CodeLlama model finetuned on performance-conditioned data (denoted as \piecond).

\para{Evaluating performance improvement of code optimization model.}
LLMs have been extensively used in code optimization in the recent works~\cite{shypula-iclr24,gao-icse24,cummins-arxiv24}, however, oftentimes they rely on a limited set of tests that were created to evaluate correctness when evaluating performance improvement.
But those correctness tests might not be stressing enough to reveal the difference between a slow program and a fast, optimized program.
To investigate how stress tests generated by \tool can help evaluate the performance improvement of code optimization models, we adapt the state-of-the-art code optimization technique~\cite{shypula-iclr24} to our framework. 

We pick the most powerful models finetuned by \citet{shypula-iclr24}, 13B CodeLlama model finetuned on 
(1) HQ + self-play augmented data (denoted as \piehq), 
(2) performance-conditioned data (denoted as \piecond), and 
(3) the entire PIE dataset unconditionally (denoted as \pieuncond) to optimize C++ programs.

We use the slowest five inputs produced by \tool, default tests (public + private tests), and the slowest five inputs from default tests.
We then select solutions using similar criteria (detailed in Appendix~\ref{sec:utility_filtering}, and got 995 solutions from 199 problems. We follow the settings in \cite{shypula-iclr24} to evaluate the speedup (time-wise and instruction-count-wise) and ratio of solutions that are optimized (speedup higher than 1.1x).

As shown in Table~\ref{tab:pie-experiment}, using \tool tests can reveal higher performance improvement than other input sets in most metrics.
For example, with the other three input sets \piehq is showing speedup (time-wise) lower than 1x, which leads to misleading conclusion that this model is doing poor at speedup.
But when using our tests the speedup reaches 1.18x, exhibiting better capability in terms of optimization. We argue it's because the measurement of execution time is sensitive to noise, especially when the tests are not stressing.
When executing more stress tests the effect of noise is significantly reduced.
%  
Besides, \defaultslowfive shows similar performance with \defaultall, indicating even the slow default tests fail to make optimized solutions stand out.
To conclude, stress tests are required for evaluating efficiency in code editing, and they can reveal performance difference better than default tests that are created for evaluating correctness.


\iffalse
\begin{table}[!ht]
  \caption{Average and median instruction counts across all tested programs when running top-10, 5, 3, and 1 slowest inputs.}
  \label{tab:instruction-count}
  \begin{tabular}{lrr}
    \toprule
    Technique&Average&Median\\
    
    \midrule
    \rowcolor[gray]{0.8}
    \multicolumn{3}{c}{\textbf{Top 10 slowest inputs}}\\
    \tool & $1.389$ $\times$ $10^9$ & $0.591$ $\times$ $10^9$ \\
    \evalperfslow & $0.944$ $\times$ $10^9$ & $0.010$ $\times$ $10^9$ \\
    \evalperfrandom & $0.803$ $\times$ $10^9$ & $0.009$ $\times$ $10^9$ \\
    \directprompting & $0.487$ $\times$ $10^9$ & $0.004$ $\times$ $10^9$ \\
    
    \midrule
    \rowcolor[gray]{0.8}
    \multicolumn{3}{c}{\textbf{Top 5 slowest inputs}}\\
    \tool & $1.965$ $\times$ $10^9$ & $0.558$ $\times$ $10^9$ \\
    \evalperfslow & $1.039$ $\times$ $10^9$ & $0.015$ $\times$ $10^9$ \\
    \evalperfrandom & $0.848$ $\times$ $10^9$ & $0.013$ $\times$ $10^9$ \\
    \directprompting & $0.558$ $\times$ $10^9$ & $0.08$ $\times$ $10^9$ \\

    \midrule
    \rowcolor[gray]{0.8}
    \multicolumn{3}{c}{\textbf{Top 3 slowest inputs}}\\
    \tool & $2.736$ $\times$ $10^9$ & $0.585$ $\times$ $10^9$ \\
    \evalperfslow & $1.067$ $\times$ $10^9$ & $0.021$ $\times$ $10^9$ \\
    \evalperfrandom & $0.863$ $\times$ $10^9$ & $0.020$ $\times$ $10^9$ \\
    \directprompting & $0.590$ $\times$ $10^9$ & $0.008$ $\times$ $10^9$ \\

    \midrule
    \rowcolor[gray]{0.8}
    \multicolumn{3}{c}{\textbf{Top 1 slowest inputs}}\\
    \tool & $2.791$ $\times$ $10^9$ & $0.644$ $\times$ $10^9$ \\
    \evalperfslow & $1.122$ $\times$ $10^9$ & $0.027$ $\times$ $10^9$ \\
    \evalperfrandom & $0.892$ $\times$ $10^9$ & $0.027$ $\times$ $10^9$ \\
    \directprompting & $0.638$ $\times$ $10^9$ & $0.09$ $\times$ $10^9$ \\
  \bottomrule
\end{tabular}
\end{table}

\begin{table}[!ht]
  \caption{Average and median running time across all tested programs when running top-10, 5, 3, and 1 slowest inputs.}
  \label{tab:app}
  \begin{tabular}{lrr}
    \toprule
    Technique&Average (ms) & Median (ms)\\
    
    \midrule
    \rowcolor[gray]{0.8}
    \multicolumn{3}{c}{\textbf{Top 10 slowest inputs}}\\
    \tool & $287$ & $54$ \\
    \evalperfslow & $244$ & $105$ \\
    \evalperfrandom & $188$ & $43$ \\
    \directprompting & $127$ & $41$ \\
    
    \midrule
    \rowcolor[gray]{0.8}
    \multicolumn{3}{c}{\textbf{Top 5 slowest inputs}}\\
    \tool & $367$ & $53$ \\
    \evalperfslow & $263$ & $108$ \\
    \evalperfrandom & $200$ & $45$ \\
    \directprompting & $141$ & $43$ \\

    \midrule
    \rowcolor[gray]{0.8}
    \multicolumn{3}{c}{\textbf{Top 3 slowest inputs}}\\
    \tool & $474$ & $54$ \\
    \evalperfslow & $272$ & $110$ \\
    \evalperfrandom & $204$ & $46$ \\
    \directprompting & $146$ & $44$ \\

    \midrule
    \rowcolor[gray]{0.8}
    \multicolumn{3}{c}{\textbf{Top 1 slowest inputs}}\\
    \tool & $485$ & $56$ \\
    \evalperfslow & $292$ & $113$ \\
    \evalperfrandom & $215$ & $49$ \\
    \directprompting & $158$ & $45$ \\
  \bottomrule
\end{tabular}
\end{table}

\begin{table}[ht!]
  \caption{Average and median CV for running time and \# instructions, respectivelly across all programs.}
  \label{tab:app}
  \begin{tabular}{lrrrr}
    \toprule
    Technique&\multicolumn{2}{c}{Running time}&\multicolumn{2}{c}{\# Instructions} \\
             &Avg.&Med.&Avg.&Med. \\
    \midrule
    \tool & 13\% & 12\% & 0.03\% & $<$0.01\% \\
    \evalperfslow & 12\% & 11\% & 0.05\% & $<$0.01\% \\
    \evalperfrandom & 12\% & 11\% & 0.04\% & $<$0.01\% \\
    \directprompting & 12\% & 12\% & 0.02\% & $<$0.01\% \\
    

  \bottomrule
\end{tabular}
\end{table}

\fi

\iffalse

\subsection{Dataset}
\label{sec:data}

% \para{Data set} 

We use the CodeContest dataset~\cite{alphacode}---a dataset primarily used for training machine learning models for code generation and analysis.
The CodeContests dataset is a comprehensive collection of competitive programming problems obtained from multiple platforms (e.g., \codeforces, AtCoder, and CodeChef). The training set alone comprises of over 13,000 problems, each paired with both correct and incorrect human submissions implemented in a variety of programming languages (C, C++, Python, and Java). 
These problems are representative of different difficulty levels and cover diverse algorithmic and data-structure challenges. 
Alongside problem statements and constraints, each entry typically includes sample test cases that facilitate automated evaluation of solution correctness.

The dataset structure is designed to provide multiple solutions per problem, often ranging from dozens to hundreds of both correct and incorrect submissions. 
Each solution is directly tied to a set of test inputs and outputs. 
In many cases, problems feature multiple test inputs---dozens to hundreds---to cover different edge cases and typical scenarios, helping ensure that generated or analyzed code is exposed to a variety of input-output patterns.

The goal of our framework is to generate inputs that expose performance bottlenecks in the programs under test.
As such, we filter out programs from our data set that are unlikely to show noticeable slowdown under challenging inputs.

%The goal of our pipeline is to generate inputs that surface performance bottlenecks for the programs under test.
%Yet even with the most challenging inputs, some short-running programs might not exhibit performance degradation due to the noise and measurement biases discussed above.

% As such, we apply a series of filters to remove programs that might not show improvement regardless of the quality of the inputs.
%

\para{Output agreement}. 
AlphaCode tests are not guaranteed to follow problem constraints (e.g., maximum input size)~\cite{alphacode} which could lead to undefined behavior when solutions run some of those non-compliant inputs.
Thus, for every test input we require that at least 95\% of the programs give the exact same answer.
We discard the problems for which this does not hold.

\para{Sufficient computation}. Profiling short-running programs is challenging and prone to measurement errors~\cite{,}.
Thus, we discard problems that are solved by short-running programs, namely if they contain programs that run no more than $10,000$ instructions on any test input.

\para{Sufficient data}. We discard problems that are solved by less than five programs.
Additionally, we discard problems that have less than come with less than five test inputs.

\para{Running time variation ranking}. Intuitively,
We start by measuring the running time variability of the programs solving a particular problem. 
For each problem, we run the programs that solve it executing AlphaCode tests~\cite{alphacode}.
We then measure the coefficient of variation (CV) per problem, and rank problems from the highest CV.
% We then pick the top 100 problems with the highest CV.

The intuition behind this filtering is that programs with approximately the same running time likely indicate less distinguishable inefficiencies in the code.



After applying the above filters, we obtained 933 problems. We further rank the problems based on CV and selected the top 300 problems as our final set.
Note that in the scenario of coding problems, many performance-characterizing constraints are "trivial" rather than "non-trivial", in the sense that the dominating constraints in terms of performance are oftentimes size of the inputs, \ie, the larger the input, the slower the program will run. Driven by curiosity, we want to understand specifically how \tool is good at identifying "non-trivial" constraints (that are not size-related). To this end we further picked a subset of \textbf{xxx} problems based on the following criteria:

\textbf{filters}

The subset is denoted as \benchsubset.

\fi

==> methodology_old.tex <==
\section{Methodology}



% To tackle this research problem, we developed \tool, a pipeline that combines traditional execution monitoring, fuzzing, and large language models to synthesize pc-constraints for a program under test ($\mathcal{P}$) and, ultimately, generate performance-exercising inputs.
Figure~\ref{fig:wedge-workflow} shows the workflow of \tool, \ie, given a program under test ($\mathcal{P}$), how it generates the performance stressing inputs.
% Our pipeline works in three stages.
It is powered by coverage-guided fuzzing, a technique that has been shown to be effective in test generation and bug detection~\cite{zhu2022fuzzing,bohme2017directed,fioraldi-woot20}.
The pipeline works in the following three stages.

% .

% \para{Input Pair Mining. }
% \tool starts by identifying a pair of \textit{contrasting} inputs whose execution profiles present significant differences while having some similarity.
% It first runs $\mathcal{P}$ against a set of user-provided tests, \eg, existing tests provided by the dataset to test correctness (\circled{1}).

\subsection{Execution Feedback Collection}

% 
We first collect high-quality contrastive execution feedback (fast and slow executions) in order to help the \llm to reason about performance constraints in the next stage.
This is achieved in two steps.

\para{Contrastive input pair mining.} In this step, \tool runs $\mathcal{P}$ against a set of user-provided tests, \eg, existing correctness tests provided by the dataset (\circled{1}).
% While running these tests, \tool collects line-level execution profiles (\eg, coverage and hit count) and the number of executed assembly instructions.
While running these tests, \tool collects the number of executed hardware instructions.
% We use number of instructions, denoted as $|I|$, to reflect the cost of executions, as instruction count is more reliable and less susceptible to noise as shown in Section~\ref{sec:quantitative_results}.
We use number of instructions, denoted as $|I|$, to reflect the cost of executions, as instruction count is more reliable and less susceptible to noise as demonstrated by \citet{liu-colm24}.

\tool pairs up the inputs in twos, and calculate the similarity of two inputs.
The similarity is the sum of \textit{match ratio} (number of common array elements / length of the shorter input array) and \textit{Jaccard similarity}~\cite{niwattanakul2013using}.
Then the input pairs are ranked by the similarity.
For input pairs with the same similarity, we further rank them by execution cost ratio between the number of instructions of slow input and that of fast input.
\tool selects the top-1 input pair, denoted as $(i_{s},i_{f})$.
The insight of using contrasting input pairs to inspire constraint reasoning comes from \textit{delta debugging}~\cite{zeller-tse02}. Delta debugging isolates bugs by systematically comparing and narrowing down the difference (delta) between the passing case and the failing case, to find the minimized set of bug-inducing circumstances. By providing the similar-but-different input pairs along with the execution feedback, \llm can ``delta-debug'' by pinpointing the differences between inputs and feedback to understand why the slow input makes the program run slow.

\para{Profiling feedback collection.}
After obtaining the potentially promising input pair, \tool executes $\mathcal{P}$ with ${i_{s}}$ and ${i_{f}}$ and collects feedback (coverage and hit count) of the executions (\circled{2}) $F_{s}$ and $F_{f}$, respectively.
Such feedback has been shown to be helpful in debugging~\cite{lin_icse17}.
Our insight is that it can help \llm diagnose performance as well and inspire the \llm to better reason about performance constraints.
The insight is similar to classic debugging ideas like delta debugging~\cite{zeller-tse02} and statistical debugging~\cite{zheng_icml2006}, where developers identify correlations between multiple input-result pairs to debug.
Powered by LLMs, our approach does not require human intervention thus can be fully automated.



% \para{PC-constraint synthesis.} In this stage, \tool starts by identifying a pair of \textit{contrasting} inputs whose execution profiles present significant differences while having some similarity.
% In our current setup, ``significant'' means that one input executes at least 20\% instructions more than the other (\circled{3}).
% Next, it then annotates $\mathcal{P}$ with the two execution line-level profiles (coverage and hit count information), adds the contrasting inputs, along with the problem specification and asks the \llm to identify potential pc-constraints.
% It further instructs the \llm to output these pc-constraints in natural language as well as in the form of C-style assertions, and integrate those assertions into an ``instrumented'' version of $\mathcal{P}$, (\circled{4}).

\subsection{Performance-characterizing constraint Synthesis}
% In this stage, \tool 1) generates the constraints (in natural language) based on contrasting execution feedback, 2) prompts the \llm to implement the constraint checkers (based on the natural language constraints) to the program (as fuzz driver) to facilitate coverage-guided fuzzing.
In this stage, \tool generates the constraints (in natural language) in the first step.
In the second step, it prompts the \llm to implement the constraint checkers based on the natural language constraints and insert them to the fuzz driver.

\para{Performance-characterizing reasoning.}
% \tool first constructs a comprehensive prompt containing the problem statement, solution program, contrasting inputs, the profiling feedback information, and multiple manually-crafted constraints as few-shot examples.
% Then it prompts the \llm with CoT few-shot learning~\cite{wei-nips22} to explicitly reason about and generate the performance-characterizing constraints by comparing the contrasting inputs $i_{s}$ \vs $i_{f}$ and their feedback ${F_{s}}$ \vs ${F_{f}}$, denoted as $\mathcal{C_P}$.
\tool first constructs a comprehensive \textit{performance reasoning prompt template} that contains the problem statement, solution program, contrasting inputs, the profiling feedback information, and multiple manually-crafted constraints as few-shot examples.
The template explicitly instructs the LLM to reason about performance constraints in multiple phases, as shown in Figure~\ref{fig:motivating}.
In Phase 1, the LLM needs to identify expensive or inefficient code segments.
This includes: 1) comparing line-level hit counts between the fast and slow runs, 2) pinpointing lines or functions that get significantly more hits under the slow input, and 3) infer how these lines might be interacting with data structures, loops, recursion, etc., especially as they relate to the input constraints (e.g., n <= 100).
In Phase 2, the LLM will derive performance-characterizing constraints in natural language.
By enforcing the LLM to reason about the constraints in a systematic manner with CoT few-shot learning~\cite{wei-nips22}, \tool can collect useful insights and generate high-quality constraints, denoted as $\mathcal{C_P}$, \eg Figure~\ref{fig:motivating} (green part).


\para{Constraint checker implementation.}
% \tool insert corresponding checker branches to the original program to produce the instrumented program (\circled{3}).
% \tool writes down the constraints $\mathcal{C_P}$ and the instrumented program $\mathcal{P'}$.
\tool prompts the \llm with the generated constraints and instructs it to implement the checker branches faithfully and produce the instrumented program (\circled{3}).
The instrumented program with inserted checker branches, denoted as $\mathcal{P'}$, will be used as the fuzz driver.


% \noindent
% \begin{minipage}{0.48\textwidth}
% \begin{lstinputlisting}
% [language=Python, numbers=left, caption={\tool synthesized constraint-aware fuzzing mutator for Problem 633A}, label={lst:p633a-wedge}, escapechar=!<>, lineskip=-1pt]
% {listings/633_A_solutions_0622_wedge_mutator.py}
% \end{lstinputlisting}
% \end{minipage}
% \hfill
% \begin{minipage}{0.46\textwidth}
% \begin{lstinputlisting}
% [language=Python, numbers=left, caption={\evalperfslow synthesized generator for Problem 633A}, label={lst:p633a-evalperfslow}, escapechar=!<>, lineskip=-1pt]
% {listings/633_A_evalperf_slow_gen.py}
% \end{lstinputlisting}

% \begin{lstinputlisting}
% [language=Python, numbers=left, caption={\evalperfrandom synthesized generator for Problem 633A}, label={lst:p633a-evalperfrandom}, escapechar=!<>, lineskip=-1pt]
% {listings/633_A_evalperf_random_gen.py}
% \end{lstinputlisting}
% \end{minipage}


\subsection{Constraint-Aware Input Mutation}
In this stage, \tool launches coverage-guided fuzzing on the fuzz driver ($\mathcal{P'}$) to generate performance-stressing inputs.

\begin{wrapfigure}[29]{r}{0.57\textwidth}
\begin{center}

\vspace{-2em}
\begin{lstinputlisting}
[language=C++, numbers=left, caption={A constraint checker for Problem 633A}, label={lst:p633a-constraint-checker}, escapechar=!<>, lineskip=-1pt, xleftmargin=1em, framexleftmargin=1.5em]
{listings/633_A_solutions_0622_checker_2.cpp}
\end{lstinputlisting}
% \vspace{-1em}
\begin{lstinputlisting}
[language=Python, numbers=left, caption={\tool synthesized constraint-aware fuzzing mutator for Problem 633A}, label={lst:p633a-wedge}, escapechar=!<>, lineskip=-1pt, xleftmargin=1em, framexleftmargin=1.5em]
{listings/633_A_solutions_0622_wedge_mutator.py}
\end{lstinputlisting}
\end{center}
\end{wrapfigure}

% \begin{wrapfigure}{r}{0.54\textwidth}
% \begin{minipage}{0.50\textwidth}
% \begin{lstinputlisting}
% [language=Python, numbers=left, caption={\evalperfrandom synthesized generator for Problem 633A}, label={lst:p633a-evalperfrandom}, escapechar=!<>, lineskip=-1pt]
% {listings/633_A_evalperf_random_gen.py}
% \end{lstinputlisting}
% \end{minipage}
% \end{wrapfigure}

\para{Constraint-aware mutator generation.}
\tool uses \afl as its fuzzing engine. 
% In this stage, given the instrumented program, \tool uses \afl as its fuzzing engine. 
% It, once again, relies on the \llm to generate mutators, given the instrumented program $\mathcal{P}$ and the natural language description of the pc-constraints (\circled{5}).
Note that the default mutator of AFL++ targets at binary fuzzing (including operations like bitflip, byteflip, crossover \etc), having no knowledge of input validity constraints, thus could generate mostly invalid inputs.
% 
Fortunately, \afl supports using user-provided customized mutator~\cite{fioraldi-woot20}.
% This is one of the major updates from AFL.
Therefore, \tool prompts the \llm with both validity constraints (\ie, the problem statement) and performance constraints to produce validity-and-performance-aware mutators (\circled{4}).
% Note that this was already generated by the \llm in the previous stage.
For example, Listing~\ref{lst:p633a-constraint-checker} is another constraint checker for problem 633A in addition to 
\codeIn{check\_gcd\_constraint} in Figure~\ref{fig:motivating}.
Listing~\ref{lst:p633a-wedge} is a mutator generated for problem 633A.
The mutator incorporates both validity constraints (\eg $1 \leq a, b \leq 100, 1 \leq c \leq 10000$) and performance constraints (\ie \codeIn{check\_close\_values\_constraint} in Listing~\ref{lst:p633a-constraint-checker}, \ie difference between a and b should be less than 5, either a or b should not be the divisor of c), thus can continuously produce diverse constraint-satisfying inputs in fuzzing.
% While the generators generated by \evalperf or \directprompting fail to catch the complex performance constraints, as shown in Listing~\ref{lst:p633a-evalperfrandom}, Listing~\ref{lst:p633a-evalperfslow}, and Listing~\ref{lst:p633a-directprompting}.
% 
While the generator produced by the state-of-the-art technique \evalperf fails to catch the complex performance constraints, as shown in Listing~\ref{lst:p633a-evalperfrandom}.

\begin{wrapfigure}[10]{r}{0.54\textwidth}

\begin{center}
\vspace{-2em}
\begin{lstinputlisting}
[language=Python, numbers=left, caption={\evalperfrandom synthesized generator for Problem 633A}, label={lst:p633a-evalperfrandom}, escapechar=!<>, lineskip=-1pt]
{listings/633_A_evalperf_random_gen.py}
\end{lstinputlisting}
\end{center}
\end{wrapfigure}



% 
\para{Constraint-guided fuzzing.}
Once mutators are generated, it launches fuzzing campaign using the mutators for one hour on multiple instrumented programs (no more than 10 for our experiments) in parallel, collecting all tests generated by \afl (\circled{5}).



However, not all generated tests strictly conform to the validity constraints.
We prompt the \llm with the problem statement to produce an input validator to filters out likely invalid inputs (detailed in ).
Plus, \tool will rely on the consistency check to further reduce invalid inputs, \ie, if different correct solutions in the dataset calculate inconsistent outputs (we use the threshold of 5\%) for an input, the input will be discarded.
After two-steps filtering, the remaining tests are considered valid and aggregated into a benchmark called \bench (\circled{7}).

\iffalse
\subsection{Execution Profiling}

We begin by running the program $\mathcal{P}$ on a corpus of user-provided tests (\eg, tests provided in datasets in our experiment) to collect performance and coverage profiles.
Specifically, for every test we record execution time and the (program) line-level number of (retired) instructions.

Once \tool has profiled each test, it extracts pairs of ``contrasting inputs''---pairs of ``fast'' vs. ``slow'' test cases whose line-level hit counts differ by a specified threshold (20\%, in our experiments) while sharing similarity.
This ensures that \tool finds test pairs indicative of a potential performance bottlenecks, since program statements that consume disproportionately more instructions or time can signal inefficiencies.

\subsection{PC-constraint Synthesis}

Equipped with test-level performance profiles and a set of contrasting inputs, our \tool then implements \textit{contrastive performance-characterizing constraint generation}. 
Specifically, we provide the model with $\mathcal{P}$ annotated with line-level coverage and hit count information, along with the pair of contrastive inputs, and the problem description.
We then ask the model to synthesize PC-constraints based on this information.

The language model outputs these constraints in two formats: natural language descriptions and C-style assertions. 
These constraints are then embedded into the program as additional branch instructions. 
By integrating these new performance branches, the program’s execution space is partitioned into distinct regions: a ``regular'' performance region and a ``slow'' path that explicitly exercises inefficient code fragments.

The key insight behind our approach is to guide the model in finding conditions that may increased execution time by focusing its attention on what separates a significantly faster run from a slower one. 
This method shifts the emphasis from broad coverage to specific regions of interest that are more likely to exhibit performance bottlenecks.

Moreover, our technique decouples ``condition generation'' from ``specification constraints''. 
Put differently, pc-constraints attempt to capture \textit{why} and \textit{when} a particular code region slows down rather than focusing on generic \lengthstressing inputs. 
Asking the model to generate performance-exercising inputs directly can determine the model to focus on conceptual and generic performance pitfalls (e.g., extensive computation and resource utilization) while de-prioritizing more nuanced inefficiencies that can otherwise be revealed by specific input patterns like partially sorted arrays or unusual graph topologies.

% Iterative prompting---repeatedly ask the model to refine its answer---suffer from similar shortcomings.
% Language models can get stuck in local minima, repeat flawed or incomplete logic, or run into context window limitations. 
% Moreover, programs could have multiple performance bottlenecks, yet iterative prompting might fixate on one recognized issue and repeatedly refine it, neglecting others.

Lastly, while we focus on CPU-bound examples, the same constrastive framing generalizes to memory, network, or I/O-intensive code. 
If an execution path sees a drastic coverage or usage jump with a small change in input, the model can capture that condition as a pc-constraint.
We thus argue that our approach scales across different domains and programming languages, using consistent logic: show coverage differences which leads to generating a slowdown condition which leads to discovering a performance bottleneck.


\subsection{Fuzzing}

With the program now instrumented with embedded pc-performance constraints as C-style assertions, the next stage leverages fuzzing to generate performance-exercising inputs.
The embedded constraints guide the fuzzer toward exploring specific execution paths that are suspected of containing performance bottlenecks.

\tool relies on the \afl as our fuzzing engine, yet relies on language models to craft customized mutators.
The standard mutators provided by \afl are often insufficient for generating inputs that adhere to the nuanced input constraints of our programs. 
To address this, we developed an iterative mutator synthesis process. 
In this process, the language model is prompted to generate custom mutators based on the problem description and the natural-language description of the pc-constraints, offering a more focused approach compared to generic, off-the-shelf mutators.

To generate customized mutators, the model is provided with both the instrumented program and the natural language descriptions of the constraints. This approach ensures that the mutators are specifically tailored to create inputs that activate the embedded performance branches, thereby targeting the “slow path” regions of the program.

After generating mutators, \tool launches a time-bound fuzzing campagin (one hour, in our experiments) during which \afl uses the customized mutators to generate new test cases.
All tests produced by the fuzzer are collected and labeled as performance-exercising tests. These tests are subsequently aggregated into our performance benchmark, \bench, which serves as a repository of inputs that exercise the identified performance bottlenecks.
\fi


\iffalse

\subsection{Iterative Mutator \& Validator Generation}
\para{Mutator Synthesis}. Although \afl~\cite{fioraldi-woot20} has shown superior performance in terms of coverage-guided test input generation, it is not ready to use off-the-shelf. The default mutators of \afl engine are optimized for compact data formats - say, images, multimedia, compressed data, \etc, supporting operations like flipping bits, inserting bytes, changing bytes, \etc But such byte-level mutators will produce a lot of invalid inputs that violate input constraints of the coding problems. Instead of using the default mutators, we rely on the \textit{custom mutators} interface of \afl, which allows user to specify a customized Python or C++ mutator script as the mutator engine. 
We prompt the model by feeding problem description, summarized constraints, \afl provided mutator example, \etc Note that different from \evalperf and \directprompting style \textit{generator synthesis}, \textit{mutator synthesis} is more challenging since in addition to making sure the mutated input follow the input constraints, it also needs to be robust enough to mutate inputs in various shapes. To this end, we propose to use an iterative mutator generation approach. 
The intuition comes from recent works~\cite{chunqiu-issta24} showing LLMs are good at fixing programs conversationally. For each generated mutator, we launch a dry run for three minutes. 
If the dry run successfully generates a bunch of test inputs, the mutator is labeled as ``pass'', otherwise, we add the failing message such as ``IndexError: list assignment index out of range'' to the conversation and ask the \llm to fix the issue. The prompting-and-dry-run loop terminates when a good mutator is produced or five rounds have been tried.

\para{Input Validator Synthesis and Consistency Check}
Both fuzzing and prompting-based generator generation can produce a large amount of test inputs. 
However, the generated inputs might violate the input format or specifications in the problem description. To tackle this problem, \cite{liu-neurips23} adopted a \textit{programming by contract} philosophy by manually annotating function pre-conditions in the form of code assertions (\eg, \codeIn{assert n > 0}) to ensure the test inputs for the function are well-formed. 
However, manual annotation is known to be error-prone and expensive~\cite{brants-emnlp07}. On the other hand, synthesizing a validator is generally challenging as there's no ground truth. Luckily, we can utilize the test cases (which are labeled as correct by authors) in the dataset as the source of harness, following the paradigm of Programming By Example (PBE), \ie, a good validator should not label any valid inputs as invalid. Specifically, we iteratively prompt the \llm to generate a validator Python script and execute it on the ``public'' and ``private'' test cases. If some tests fail, we append the failing message to the conversation and ask the model to fix the validator, until all tests pass or it reaches the retry limits. Note that this approach does not ensure the correctness of the validators as the synthesis problem is generally undecidable, but it gives us higher confidence on the reliability of the validors.

In addition to the generated validator, we introduce the \textit{consistency check} to further filter out invalid inputs. For each generated input, we execute all correct solutions under the input and check whether 95\% of them are consistent. Inputs leading to over 5\% inconsistent results will be discarded. The intuition is that a well-formed input should be processed correctly by all correct solutions.

We apply the validators and consistency check to all techniques to ensure fairness.

% \begin{itemize}
%     \item For each problem, we run each program over the AplhaCode test suite 
%     \item We then compute the coefficient of variation over the execution times obtained after running the AlphaCode test suite
%     \item We keep the top XXX problems in terms of highest CV
%     \item The key insight behind this strategy is to filter out problems whose solutions might not exhibit much "running time" diversity. Programs with approximately the same running time likely indicate less distinguishable inefficiencies in the code. 
%     \item This is somewhat a pathology of the CodeContest data set. The data set includes programs that solve competition puzzles, programs that have to adhere to strict running time constraints. To get maximum points, The programs need to implement optimal or near-optimal solutions and run within the running time restrictions.
% \end{itemize}

% 
% \begin{itemize}
%     \item LLMs might sometimes propose unrealistic or invalid inputs because they lack actual runtime checks to confirm correctness or code reachability. A naive direct-input approach might yield a random large input that does not trigger the actual inefficienc code path.
%     \item Simply telling the \llm “generate a slow input” can lead to plausible-sounding but performance-irrelevant inputs.  
%     \item The \llm focuses on the conceptual performance pitfalls (e.g., high complexity, pathological data distributions). However, asking the \llm to generate performance-related constraints produces more nuanced inputs: e.g., “if (array sorted ascending and size > 10,000) ...”. So this constraint-generation approach approach can highlight that the true inefficiency is triggered only when the array is both large and partially sorted.
%     \item With constraints integrated into the program, any fuzzed input that triggers the “if” statement provides immediate feedback that performance is indeed being pushed into a problematic edge case.
% \end{itemize}

% 
% \begin{itemize}
%     \item Contrasting examples explicitly signal to the \llm that it should focus on performance, because the ``fast'' vs. ``slow'' input conveys how certain inputs trigger compleixty issues.
%     \item Contrasting examples naturally focus the \llm's reasoning around what changed in the execution of the original program.
%     \item With generic prompting approahces \llm might answer with generic inputs (e.g., large input size) that might not meaningfully stress performance
%     \item Contrasting examples generalize across domain- or language-specific issues, as the same “slow vs. fast” framing can apply to time complexity (running time), resource utilization (memory, network bandwidth), I/O-bound differences, etc. 
% \end{itemize}



\subsection{Evaluation Setup}

% \subsubsection{Dataset Collection}
% Discussed in 3.1
% \textbf{Data filtering.} 
\subsubsection{Baselines}
\para{\evalperf}. \cite{liu2024evaluating} proposed to apply few-shot prompting with Chain of Thoughts (CoT) for input generator synthesis (denoted as \sas) to generate performance-excercising inputs. \evalperf assumes the execution cost of a problem is determined by the ``scale'' of the problem, thus \evalperf introduces a ``scale factor'' as the input to the input generator function. \evalperf then samples scale factors from 1, doubling it round by round until an input hits a time or memory limit on any validated solution. Note that \evalperf requires one example solution to the problem in the prompt. It was initially experimented on HumanEval dataset where one ground-truth solution is provided. While in our dataset we have multiple correct solutions per problem so we need to select one to fill in the prompt. We respectively select a random validated solution and the slowest validated solution as the example, and they are denoted as \evalperfrandom and \evalperfslow.

\para{\directprompting}. Inspired by \evalperf~\cite{liu2024evaluating}, we also explore how directly prompting the model without any CoT, few-shot examples, scale factors, \etc, perform compared with \evalperf. \cite{jiang-ase24} and \cite{wang-arxiv24} show that LLMs exhibits impressive performance in terms of directed input generation, \ie, given a target branch in the program, instructing the \llm to generate test inputs that can cover the target branch. However, it remains unclear how well \llm can comprehend the performance-related program semantics and generate performance-excercising inputs via direct prompting. In the prompt we explicitly instruct the model to reason about the problem and generate inputs that can stress the solutions the most.

For both prompting-based techniques, we use \gpt as the backbone model and use the temperature of 0.8 following the setting in \cite{liu2024evaluating}. For each problem we generate 20 inputs to ensure diversity.

\subsubsection{Evaluating solution slow-down}
We evaluate \tool on the dataset constructed from the \codecontest dataset's training split, with a series of filters discussed in Section~\ref{sec:data}. . We primarily rely on hardware performance counter since it is easy to deploy, introduces light-weight overhead and highly reproducible.
For a given coding problem in the dataset, we only execute the solutions that were labeled as ``correct'' under all inputs. We repeat each execution for five times, so that 1) the noise from the environment can be further reduced and 2) some mislabeled incorrect solutions can be filtered out by sanity check.
We then use three metrics to evaluate the quality of the tests generated from different techniques, as shown below. Note that instead of averaging over the absolute execution time per problem, we compare all strategies on each problem individually. For each problem, we compare the scores of different techniques and record the best-performing technique for per problem per metric. In the end we show how many problems can each technique outperform all other techniques.

\para{Greatest Average Instruction Count.}

\para{Greatest Max Instruction Count.}

\para{Greatest Coefficient of Variance.}

% \subsubsection{EvalPerf vs simple prompting-based generators}
This somehow indicates that input size is not always dominating constraint

\subsubsection{Evaluating improving code optimization approaches based on execution feedback}
\cite{huang-neurips24} proposed \effilearner, utilizing execution overhead profiles to improve the efficiency of \llm-generated code. However, the approach utilizes public test cases to guide code efficiency optimization, while public tests might be not stressing enough to reveal inefficiencies of code. Driven by curiosity, we aim to leverage the stressing tests generated by \tool to improve the code optimization performance.
% To be clear, we select \placeholder slow solutions of \placeholder problems from \bench, execute the default tests and our generated tests, collect the profiling feedback correspondingly, and prompt the model to produce edited programs. Then we profile the edited programs to collect the statistics following settings of \effilearner, and compare the performance in terms of optimization.
Note that the original \effilearner explores using profiling information to improve \llm-generated code, while we adapt it to our scenario, \ie, improving slow user solutions. To this end, we extract a subset of problems and solutions from the 300 problems in \bench. Specifically, we applied the following criteria for selecting solutions:

1) Python solutions with function definitions. Because the profilers \effilearner used work on Python function level code.

2) Slow enough, containing at least 100K instructions on average and at least twice as slow as the fastest solution for the same problem. This can ensure the solution code has some complexity and there's considerable space for optimization.

3) Long enough, containing at least 50 lines. Because there might be fewer places that can potentially get optimized in smaller programs.

We select problems where at least 5 such solutions exists and select the 5 slowest solutions for each problem to consist our evaluation dataset here. In the end, we got 56 problems from \bench.

For each solution, we apply three different prompting strategies for optimization: prompting without profiling information, prompting with profiling information running \codecontest public tests, and prompting with profiling information running \tool tests, which are denoted as \textbf{\noprofile}, \textbf{\publicfiveprofile}, and \textbf{\wedgeprofile} respectively.
For models, we include the most powerful business model and open-source model at the moment this paper is written, namely OpenAI GPT-4o and DeepSeek V3. For configurations \eg, temperature, max\_length, we reused the setting in the main experiment.
Following the workflow of \effilearner, we profile the solutions written by users and prompt the model with the feedback information to optimize the solutions, then we evaluate the correctness and efficiency of the optimized solutions. Note that we only evaluate the efficiency of the correct optimized solutions, and when we compare two strategies, we evaluate on the overlapping set of solutions where both strategies produce the correct optimized solutions. We include three metrics from \effilearner work~\cite{huang-neurips24}, namely ET (Execution Time), MU (Maximum Memory Usage), TU (Total Memory Usage), and one additional metric ICT (Instruction Count). We didn't include the other three metrics (the corresponding normalized ones) from \effilearner work as we don't have the "canonical" solution in our dataset.



\subsection{Evaluting Quality of Generated Constraints}


Intuitively, the high-quality performance-characterizing constraints should be able to distinguish inputs well, \ie, inputs that satisfy the constraint should be significantly slower than the other inputs. To verify that, we first execute the inputs from \codecontest, \evalperf and \directprompting on the solutions that are inserted with constraint checks. We select these inputs since they were not generated towards our generated constraints. Then we compare the instruction counts of two groups of inputs per problem and conduct the significance test. As shown in table \placeholder, on \placeholder problems out of \placeholder problems constraint-satisfying inputs are significantly slower than the others. Overall, constraint-satisfying inputs are \placeholder slower than constraint-violating inputs.


\subsubsection{Ablation studies}

Process of generating performance-stressing inputs using \llm-generated constraints:
\begin{enumerate}
    \item Rank solutions by their baseline runtime. Gather all solutions $S_1$,$S_2$,...,$S_n$, run each program on AlphaCode official tests to measure instruction counts .
    \item Select two distinct subsets. Pick $k$ solutions/programs that run the slowest on AlphaCode tests, and $k$ solutions that run the fasted on AlphaCode test.
    \item For each of the top-k slowest solutions, craft a prompt with (a) the problem statement, (b) the solutions code, (c) fast and slow inputs, and (d) any relevant line-level hit counts for the two ``contrasting'' inputs, and then ask the \llm to generate performance constraints. We don't what to mix all solutions in the same prompt, to avoid bias in the \llm.
    \item For each solution, instrument the code with the generated constraints in the form of ``if'' statements.
    \item Run a fuzzer to generate performance-stressing input. To do this, we first use LLMs to generate a mutator specific for the problem (
    \item Re-run the code with each ``triggering'' input versus baseline AlphaCode tests to measure performance difference in terms of instruction counts.
\end{enumerate}

For the evaluation, we compare:

\begin{enumerate}
    \item EvalPerf
    \item Fuzzing for 1h
    \item \llm-only \#1: ask \llm to synthesize an input generator given only the problem statement
    \item \llm-only \#2: ask \llm to synthesize an input generator given the problem statement and the the top-k slowest solutions
    \item \llm-only \#3: ask \llm to synthesize an input generator given the problem statement, one of the top-k solution and a fast/slow input pair 
    \item WorkBench (our approach/tool)
\end{enumerate}

\fi

==> related_work.tex <==
\section{Related Work}
% DPE aims to evaluate code generation models while we focus on code editting scenario.
% dataset and code generation benchmarks
% AlphaCode (Li et al., 2022) leverages language models to generate solutions to competitive programming problems in natural language, but it does not attempt to improve the performance of existing solutions.

%baselines: evalperf

%baselines: fuzzing

\subsection{Code Generation Benchmarks}
Most existing code generation benchmarks focus on the correctness aspect.
For example, APPS~\cite{hendrycks2021measuring}, MBPP~\cite{austin2021program}, HumanEval~\cite{chen2021evaluating} and EvalPlus~\cite{liu-neurips23} work on curating high-quality Python benchmarks including coding problems along with correctness tests.
HumanEval-X~\cite{zheng2023codegeex}, MultiPLe~\cite{cassano2022multipl}, and MBXP~\cite{athiwaratkun2022multi} extend the Python tasks into other programming languages.

PIE~\cite{shypula-iclr24}, EffiBench~\cite{huang-neurips24-effibench} and EvalPerf~\cite{liu-colm24} created benchmarks for evaluating code efficiency specifically.
They respectively rely on CPU simulators (Gem5~\cite{binkert2011gem5}), physical execution time and memory, and hardware performance counters~\cite{wiki:Hardware_performance_counter}.
Gem5 is known to be stable, but the overhead is significant and does not necessarily reflect the physical performance.
Physical execution time is most susceptible to the noise from environment, and the results should be interpreted with caution.
Hardware performance counters record the number of executed instructions of a program execution.
It incurs low overhead and it highly reproducible.
But it's not necessarily linearly related to physical performance.
All three metrics were used in our evaluation (for different experiments).

\subsection{Performance-Stressing Input Generation}
\citet{liu-colm24} proposed \textit{Synthesizing a Synthesizer} (SAS).
SAS prompts an LLM with CoT few-shot learning to produce a test input sampler controlled by a parameter ``scale''.
They use exponential input sampling to generate challenging but computable inputs.
\evalperf mainly generates \lengthstressing inputs, but fall short when more fine-grained requirements are necessary, as shown in our results Section~\ref{sec:quantitative_results} and prior studies~\cite{zhang_ase2011}.

Except for prompting-based techniques, there have been attempts to use traditional fuzzing/symbolic execution techniques to generate performance-stressing inputs~\cite{pestios_ccs2017,lemieux_issta2018,zhang_ase2011,burnim_icse09,chen_icse16}.
However, the symbolic execution based techniques are known to suffer from low scalability.
While the fuzzing based techniques suffers from high overhead of line-level profiling, and the search does not have good guidance, \ie, knowledge about performance summarized by the LLM, thus limiting its effectiveness.


% \subsection{Performance-characterizing Constraint}

